Delayed Geometric Discounts: An Alternative Criterion for Reinforcement Learning

The endeavor of artificial intelligence (AI) is to design autonomous agents capable of achieving complex tasks. Namely, reinforcement learning (RL) proposes a theoretical background to learn optimal behaviors. In practice, RL algorithms rely on geometric discounts to evaluate this optimality. Unfortunately, this does not cover decision processes where future returns are not exponentially less valuable. Depending on the problem, this limitation induces sample-inefficiency (as feed-backs are exponentially decayed) and requires additional curricula/exploration mechanisms (to deal with sparse, deceptive or adversarial rewards). In this paper, we tackle these issues by generalizing the discounted problem formulation with a family of delayed objective functions. We investigate the underlying RL problem to derive: 1) the optimal stationary solution and 2) an approximation of the optimal non-stationary control. The devised algorithms solved hard exploration problems on tabular environment and improved sample-efficiency on classic simulated robotics benchmarks.

==> (ICLR) RL with non geometric dicounts/Source/Classical_RL.tex <==
\section{Reinforcement Learning in infinite horizon setting}
    Consider an infinite horizon Markov Decision Process (MDP) $\mathcal{M}=\{ \mathcal{S}, \mathcal{A}, \mathcal{P}, c, \gamma, p_0 \}$, where $\mathcal{S}$ and $\mathcal{A}$ are either finite or compact subsets of respectively $\mathbb{R}^d$ and $\mathbb{R}^{d'}$, $(d, d') \in \mathbb{N}^2$, $\mathcal{P}: \mathcal{S} \times \mathcal{A} \to \Delta(\mathcal{S})$ is a state transition kernel\footnote{$\Delta(\mathcal{S})$ denotes the set of probability measures over $\mathcal{S}$}, $c:\mathcal{S}\times \mathcal{A} \to \mathbb{R}$ is a continuous non-negative cost function, $p_0 \in \Delta(\mathcal{S})$ an initial state distribution and $\gamma \in (0,1)$ is the discount factor. 
    % \vspace{-0.3cm}
    % \begin{description}
    %     \item[--] $\mathcal{S}$ is either a finite or a compact subset of $\mathds{R}^d$, for some dimension $d\in \mathds{N}$
    %     \item[--] $\mathcal{A}$ is either a finite or a compact subset of $\mathds{R}^{d'}$, for $d' \in \mathds{N}$
    %     \item[--] $\mathcal{P}$ is the state transition kernel, i.e., a continuous mapping from $\mathcal{S} \times \mathcal{A}$ to $\Delta(\mathcal{S})$, where $\Delta(\cdot)$ denotes the set of probability measures\footnote{The $\sigma$-field is always the Borel one.} over some set,
    %     \item[--] $c:\mathcal{S}\times \mathcal{A} \to \mathbb{R}$ is a continuous non-negative cost function,
    %     \item[--] $p_0 \in \Delta(\mathcal{S})$ is the initial state distribution, and $\gamma \in (0,1)$ is the discount factor.
    % \end{description} 
    A policy $\pi$ is a mapping indicating, at each time step $t \in \mathbb{N}$, the action $a_t$ to be chosen at the current state  $s_t$. The goal of reinforcement learning algorithms is to optimise the discounted costs $\mathcal{L}(\pi, r) := \mathbb{E}_{\pi, p_0}\Big[ \sum_{t=0}^\infty \gamma^t c_t \Big], c_t := c(s_t,a_t)$,
    % \begin{align*}
    %     \mathcal{L}(\pi, r) := \mathbb{E}_{\pi, p_0}\Big[ \sum_{t=0}^\infty \gamma^t c_t \Big] \quad \textit{;} \quad  c_t := c(s_t,a_t)
    % \end{align*}
    where $\mathbb{E}_{\pi, p_0}$ denotes the expectation over trajectories generated in the MDP $\mathcal{M}$, using the policy $\pi$, and initialised according to $p_0$. 
    To this end, we look for a policy that achieves the optimal value function $V^*:\mathcal{S} \to \mathbb{R}$ defined as $V^*(s) = \min_{a_0, a_1, ... }\mathbb{E}_{\pi}\Big[\sum_{t=0}^\infty \gamma^t c_t \Big| s_0=s \Big]$. %and the state-action value function $Q^\pi:\mathcal{S}\times\mathcal{A} \to \mathbb{R}$ 
    % \begin{align*}
    %     V^*(s) = \min_{a_0, a_1, ... }\mathbb{E}_{\pi}\Big[\sum_{t=0}^\infty \gamma^t c_t \Big| s_0=s \Big]
    % \end{align*}
    
    The Bellman optimality principle suggests that it is possible to decomposes the optimisation into two sub problems: the current decision $(a_0)$ and all the remaining ones $(a_1,a_2,..)$. This translates into the following equation for any state $s_0\in\mathcal{S}$:
    \begin{align*}
        V^*(s_0) = \min_{a_0} \Big\{c(s_0,a_0) + \gamma \underbrace{\min_{a_1,a_2,...} \mathbb{E}_{\substack{s_{t+1}\sim \mathcal{P}(s_t,a_t)}}\Big[\sum_{t=1}^\infty \gamma^{t-1} c_t \Big]}_{\textstyle = \mathbb{E}_{s_1\sim \mathcal{P}(s_0,a_0)}[V^*(s_1)]} \Big\}
    \end{align*}
    a classical result in infinite horizon MDPs \cite{puterman2014markov} stipulates that if there exists a value function $V:\mathcal{S}\to\mathbb{R}$ and a policy $\pi^*:\mathcal{S}\to\mathcal{A}$ that verify the following:
    \begin{align}
        \pi^*(s) \in & \argmin_{a} \Big\{c(s,a) + \gamma \mathbb{E}_{s'\sim \mathcal{P}(s,a)}[V(s')] \Big\} \nonumber \\
        V(s) = & \min_{a} \Big\{c(s,a) + \gamma \mathbb{E}_{s'\sim \mathcal{P}(s,a)}[V(s')] \Big\} 
        \label{bellman-criterion}
    \end{align}
    then $\pi^*$ is an optimal control policy and $V=V^*=V^{\pi^*}$ where $V^{\pi}(s)$ is the expected discounted return of adopting the policy $\pi$ starting from the state $s$ defined as:
    \begin{align}
        V^{\pi}(s) = \mathbb{E}_{\pi, p_0}\Big[\sum_{t=0}^\infty \gamma^t c_t \Big| s_0=s \Big] = \mathbb{E}_{\substack{a\sim\pi(s) \\ s'\sim \mathcal{P}(s,a) }}\Big[c(s,a) + \gamma V^{\pi}(s')\Big].
        \label{V_bellman}
    \end{align}
    The Bellman criterion derived in Equation \eqref{bellman-criterion} proves that the optimal policy (in the sense of $\mathcal{L}$) is necessarily stationary: $\pi : \mathcal{S} \to \Delta(\mathcal{A})$.
    
    \subsection{Solving the geometrically discounted RL problem} 
        Value-based RL algorithms optimise $\mathcal{L}$ by looking for a policy that satisfies Equation \eqref{bellman-criterion}. This class of algorithm is grounded in the policy improvement theorem \cite{sutton2018reinforcement} that guarantees the construction of a better policy given the value function of a previous one. Let $\pi:\mathcal{S}\to\mathcal{A}$ be a given policy and let $V^\pi$ be the associated value function. Consider the policy $\hat{\pi}$ defined as: 
        \begin{align}
            \hat{\pi}(s) = \argmin_a \Big\{c(s,a) + \gamma \mathbb{E}_{s'\sim \mathcal{P}(s,a)}[V^\pi(s')] \Big\}.
            \label{policy_improvement}
        \end{align}
        The policy improvement theorem guarantees that $V^\pi(s) \leq V^{\hat{\pi}}(s)$ for any state $s\in\mathcal{S}$ \cite{sutton2018reinforcement}. 
        
        This principle is used in policy iteration (and even more recent algorithms such as Soft Actor Critic \cite{haarnoja2018soft}) to learn the optimal policy. Basically, the idea is to repeat the following steps up to convergence: 
        \begin{itemize}
            \item \textbf{Policy evaluation step:} Learn the value function $V^\pi$
            \item \textbf{Policy improvement step:} Update the policy according to Equation \eqref{policy_improvement} 
        \end{itemize}
        In order to learn the value function $V^\pi$, one possibility is to to iteratively apply of the Bellman operator $T_\pi$ (from $\mathbb{R}^{\mathcal{S}}$ to $\mathbb{R}^{\mathcal{S}}$) on a given value function $V: \mathcal{S} \to \mathbb{R}$. This operator is defined as:
        \begin{align*}
            [T_{\pi}(v)](s) = \mathbb{E}_{\substack{a\sim\pi(s) \\ s'\sim \mathcal{P}(s,a) }} \Big[c(s,a) + \gamma v(s') \Big],
        \end{align*}
        This approach is viable because $T_\pi$ is a $\gamma$-contraction whose unique solution is $V^\pi$.
        
    \subsection{The average-cost RL problem} 
        One way to avoid imposing the geometric discount is to consider the average-cost framework. In this setting the goal is to optimise the following objective function: 
        \begin{align*}
            \Bar{\mathcal{L}}(\pi,c) := \lim_{T\to\infty} \frac{1}{T} \mathbb{E}_{\pi, p_0}\Big[ \sum_{t=0}^T c_t \Big] 
        \end{align*}
        One possibility to optimise this criterion is to use a policy iteration scheme with a discount factor  $\gamma=1$. Naturally, the associated Bellman operator is no longer a contraction. For this reason, this approach is only guaranteed to work in specific MDP structure (such as reccurent MDPs). 
        
        In general, the average-cost problem can be viewer as the limit of the discounted RL problem. Notably, Blackwell proved that for any MDP, there exist a critical discount $\gamma_\text{crit}<1$ such that for any discount $\gamma\in(\gamma_\text{crit}, 1)$, solving the discounted problem is equivalent to solving the average cost one: 
        \begin{align*}
            \argmin_\pi \mathcal{L}(\pi,c) = \argmin_\pi \Bar{\mathcal{L}}(\pi,c) \quad \forall \gamma\in(\gamma_\text{crit}, 1)
        \end{align*}
        However, the critical discount $\gamma_\text{crit}$ can be arbitrarily close to 1 which induces major numerical instabilities in practice.  

==> (ICLR) RL with non geometric dicounts/Source/Introduction.tex <==
 

\section{Introduction}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    % RL in infinite horizons solves geometrically discounted problems which is limited 
    In the infinite horizon setting, and without further assumptions on the underlying Markov Decision Process (MDP), available RL algorithms learn optimal policies only in the sense of the discounted cumulative rewards \citep{puterman2014markov}. While the geometric discounting is well suited to model a termination probability or an exponentially decaying interest in the future, it is not flexible enough to model alternative weighting of the returns. Consider for example settings where the agent is willing to sacrifice short term rewards in favor of the long term outcome. Clearly, for such situations, a discounted optimality criterion is limited and does not describe the actual objective function. 
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    
    % Hard exploration tasks
    This is particularly true in hard exploration tasks, where rewards can be sparse, deceptive or adversarial. In such scenarios, performing random exploration can rarely lead to successful states and thus rarely obtain meaningful feedback. Geometric discounts tend to fail in such scenarios. Consider for example the U-maze environment in Figure~\ref{fig:hard_exporation_ex}, where the reinforcement signal provides a high reward ($+1$) when reaching the green dot in the bottom arm, a deceptive reward ($+0.9$) when reaching the blue dot in the upper arm, and a negative reward ($-1$) for crossing the red corridor. If the agent is only interested in the long term returns, then the optimal control should always lead to the green dot. However, depending on the initial state, optimal policies in the sense of the discounted \rlearning problem are likely to prefer the deceptive reward due to the exponentially decaying interest in the future (Figure~\ref{fig:v_geom}).
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    % The source of the problem
    Naturally, higher discount factors are associated with optimal policies that also optimize the average returns \citep{blackwell1962discrete}, which can solve in principle the described hard exploration problem. However, in practice, such discount values can be arbitrarily close to $1$ which entails severe computational instabilities. In addition, and particularly in continuous settings or when tasks span over extremely long episodes, discount-based RL approaches are sample-inefficient and are slow at propagating interesting feed-backs to early states.
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    % Contributions
    In this paper, we generalize the geometric discount to derive a variety of alternative time weighting distributions and we investigate the underlying implications of solving the associated RL problem both theoretically and practically.
    Our contributions are twofold. First, we introduce a novel family that generalizes the geometrically discounted criteria, which we call the \emph{delayed discounted criteria}. Second, we derive tractable solutions for optimal control for both stationary and non-stationary policies using these novel criteria. 
    %\ahmed{Finally, based on Soft-Actor-Critic \citep{haarnoja2018soft}, we propose a novel algorithm that generalizes to non-geometrically discounted criteria.} 
    Finally, we evaluate our methods on both hard exploration tabular environments and continuous long-episodic robotics tasks where we show that: 
    \begin{enumerate}
        \item Our agents can solve the hard exploration problem in a proof of concept setup.
        \item Our methods improve sample-efficiency on continuous robotics tasks compared to Soft-Actor-Critic.
    \end{enumerate}
    
    Figure~\ref{fig:v_nongeom} showcases how non-geometrically discounted criteria impacts the profile of optimal value function in the U-maze example.
    \begin{figure}[h]
        \centering
        \begin{subfigure}[b]{0.31\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/corridor_reinforcement_signal_crop.png}
            \caption{}
            \label{fig:hard_exporation_ex}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.335\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/corridor_opt_v_crop1.png}
            \caption{}
            \label{fig:v_geom}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.335\textwidth}
            \centering
            \includegraphics[width=\textwidth]{Figures/corridor_opt_v_crop.png}
            \caption{}
            \label{fig:v_nongeom}
        \end{subfigure}
        \caption{\centering (a) Hard exploration problem example, (b) optimal value function of geometrically discounted \rlearning with a discount factor $\gamma=0.99$ and (c) non-geometrically discounted \rlearning.}
    \end{figure}

==> (ICLR) RL with non geometric dicounts/Source/Limitations.tex <==
\section{Limitations}  
    Despite proving to be useful in order to solve hard exploration problems in tabular settings an improve sample efficiency in continuous environments, the proposed solutions of the delayed formulation admits several limitations 
    \paragraph{Theoretical limitations:}
        % policy improvement theorem 
        On the one hand, looking for the optimal stationary solution using Algorithm \ref{D-SAC}, the policy update does not guarantee a systematic improvement in the performance. 
        
        We found out in practice that this does not entail severe performance drawback 
        % Convergence bounds with respect to the horizon H
        
    \paragraph{Algorithmic limitations:}
        % Exploding value of the Q values 
        % increased computational burden 

==> (ICLR) RL with non geometric dicounts/Source/abstract.tex <==
\begin{abstract}
    The endeavor of artificial intelligence (AI) is to design autonomous agents capable of achieving complex tasks. Namely, reinforcement learning (RL) proposes a theoretical background to learn optimal behaviors. In practice, RL algorithms rely on geometric discounts to evaluate this optimality. 
    Unfortunately, this does not cover decision processes where future returns are not exponentially less valuable.
    Depending on the problem, this limitation induces sample-inefficiency (as feed-backs are exponentially decayed) and requires additional curricula/exploration mechanisms (to deal with sparse, deceptive or adversarial rewards).
    In this paper, we tackle these issues by generalizing the discounted problem formulation with a family of delayed objective functions. We investigate the underlying RL problem to derive: 1) the optimal stationary solution and 2) an approximation of the optimal non-stationary control. 
    The devised algorithms solved hard exploration problems on tabular environment and improved sample-efficiency on classic simulated robotics benchmarks.
\end{abstract}

%%%% Previous versions 
    
    %We are interested in designing artificial agents capable of achieving lifelong and hard exploration tasks. Classic reinforcement learning (RL) approaches rely on geometrically discounted optimality criteria to learn policies. 
    %On the one hand, this does not cover decision processes where future returns are not exponentially less important. On the other hand, this is limiting in practice, as the decaying interest in future rewards is likely to exacerbate sample-efficiency, and in hard exploration scenarios, where additional curricula and exploration mechanisms are usually required to tackle the sparsity, deceptiveness or adversariality of the rewards. 
    %To circumvent these issue, we propose a novel family of non-geometrically discounted criteria. Furthermore, we derive solutions for optimal control in both stationary and non-stationary policies. We implement an instance of this novel criteria that generalizes the Soft-Actor-Critic algorithm to non-geometric discounts. We show that our methods solve the hard exploration problem in tabular environments and improve sample-efficiency in several continuous robotics tasks.
    
    
    %\ahmed{The endeavor of artificial intelligence (AI) is to design autonomous agents capable of achieving complex tasks. Namely, reinforcement learning (RL) proposes a theoretical background to learn optimal behaviors. Classic approaches in RL rely on geometric discounts (GD) to define this optimality. However, this does not cover decision processes where future returns are not exponentially less valuable. Hence, such scenarios usually suffer from sample-inefficiency and require additional curricula and exploration mechanisms. We propose an alternative family of discounted optimality criteria, named \emph{Delayed Geometric Discounts} (DGD) and show that classic GD is a particular case of DGD. This paper makes two contributions: 1) DGD, a novel family of discounted optimality criteria that uses alternative time weighting distributions; 2) Tractable solutions for optimal control for both stationary and non-stationary policies. As this paper shows, using DGD allows to solve hard exploration problems on tabular environment where classic GD fails and to improve sample-efficiency on classic simulated robotics benchmarks.}
    
    %\todo{using acronyms looked simpler than repeating the whole words, amma feel free to change that if you disagree :)} % ok, j'ai reformulé chwaya bech na3malha l3amaliya. 
    
    %\todo{Proposed two new titles. Check main file} % title 2 is good enough (y)
    
    % (V2) Artificial intelligence (\ai) strives for designing autonomous agents endowed with complex capabilities. Namely, reinforcement learning (\rlearning) proposes a theoretical background to learn optimal behaviours. However, classic approaches define this optimality with respect to the discounted cumulative returns criterion. This is particularly limiting in hard exploration environments with sparse, deceptive or adversarial reinforcement signals. In this paper, we exhibit a novel family of optimality criteria that puts more weight on future returns. Accordingly, we propose algorithmic schemes to learn optimal stationary policies and approximate the underlying control in general. As a proof of concept, we show that our agents successfully solve hard exploration problems in tabular settings. We also show that our method improves sample efficiency on classic simulated robotics environments.
    % (V1) The goal of Reinforcement Learning (\rlearning) is to find optimal control policies with respect to the discounted cumulative returns criterion. This is particularly limiting in hard exploration environments with sparse, deceptive or adversarial reinforcement signals. In this work, we investigate an alternative family of optimality criteria that puts more weight on future returns and we propose algorithmic schemes to learn the optimal stationary policy in these settings as well as approximate the underlying optimal control in general. The learned solutions successfully solved hard exploration problems in tabular setting.

==> (ICLR) RL with non geometric dicounts/Source/conclusion.tex <==
\section{Conclusion}
    Designing human-like autonomous agents requires (among other things) the ability to discard short term returns in favor of long term outcomes. 
    Unfortunately, existing formulations of the reinforcement learning problem stand on the premise of either discounted or average returns: both providing a monotonic weighting of the rewards over time. 
    
    In this work, we propose a family of delayed discounted objective functions that captures a wide range of non-monotonic time-preference models. 
    We analyse the new formulation to construct 1) the Bellman optimality criterion of stationary solution and 2) a feasible iterative scheme to approximate the optimal control. 
    The derived algorithms successfully solved tabular hard exploration problems and out-performed the sample efficiency of SAC in various continuous control problems; thus closing the gap between what is conceivable and what is numerically feasible. 

\subsubsection*{Broader Impact Statement}
    Reinforcement learning provides a framework to solve complex tasks and learn sophisticated behaviors in simulated environments. However, its incapacity to deal with very sparse, deceptive and adversarial rewards, as well as its sample-inefficiency, prevent it from being widely applied in real-world scenarios. We believe investigating the classic optimality criteria is crucial for the deployment of RL. By introducing a novel family of optimality criteria that goes beyond exponentially discounted returns, we believe that we take a step towards more applicable RL. In that spirit, we also commit ourselves to releasing our code soon in order to allow the wider community to extend our work in the future. 


==> (ICLR) RL with non geometric dicounts/Source/contribution.tex <==
\section{Reinforcement Learning with non geometric discount}
    Consider an infinite horizon Markov Decision Process (MDP) $\mathcal{M}=\{ \mathcal{S}, \mathcal{A}, \mathcal{P}, r, \gamma, p_0 \}$, where $\mathcal{S}$ and $\mathcal{A}$ are either finite or compact subsets of respectively $\mathds{R}^d$ and $\mathds{R}^{d'}$, $(d, d') \in \mathds{N}^2$, $\mathcal{P}: \mathcal{S} \times \mathcal{A} \to \Delta(\mathcal{S})$ is a state transition kernel\footnote{$\Delta(\mathcal{S})$ denotes the set of probability measures over $\mathcal{S}$}, $r:\mathcal{S}\times \mathcal{A} \to \mathds{R}$ is a continuous reward function, $p_0 \in \Delta(\mathcal{S})$ an initial state distribution and $\gamma \in (0,1)$ is the discount factor. 
    A policy $\pi$ is a mapping indicating, at each time step $t \in \mathds{N}$, the action $a_t$ to be chosen at the current state  $s_t$. The goal of geometrically discounted reinforcement learning algorithms is to optimize the discounted returns:
    \begin{align*}
        \mathcal{L}(\pi, r) := \mathds{E}_{\pi, p_0}\Big[ \sum_{t=0}^\infty \gamma^t r_t \Big] \quad \textit{;} \quad  r_t := r(s_t,a_t)
    \end{align*}
    where $\mathds{E}_{\pi, p_0}$ denotes the expectation over trajectories generated in $\mathcal{M}$ using the policy $\pi$ and initialised according to $p_0$. 
    
    In this section, we present our methods. First, Section~\ref{sec:non_geom_criteria} introduces our delayed discounted family of optimality criteria. Then, Section~\ref{sec:optimal_stationary} investigates the optimization of the linear combination of this new family in the context of stationary policies. Finally, Section~\ref{sec:optimal_control} generalizes the optimal control to non-stationary policies.
    % In this section, we start by introducing a family of optimality criteria that generalises the geometric discount and then we construct tractable algorithmic approaches to solve the underlying problems. 
    
    \subsection{Beyond the geometric discount: A delayed discounted criterion}
    \label{sec:non_geom_criteria}
        We propose to investigate a particular parametric family of optimality criteria that is defined by a sequence of discount factors.
        For a given delay parameter $D\in\mathds{N}$, we define the discount factors $\gamma_d \in(0,1)$ for any integer $d\in[0,D]$ and we consider the following loss function:
        \begin{align}
            \mathcal{L}_D(\pi, r) := \mathds{E}_{\pi, p_0} \Big[ \sum_{t=0}^\infty \Phi_D(t) r_t \Big] 
            \quad \textit{where} \quad 
            \Phi_D(t) := \sum_{\substack{ \{a_d \in \mathds{N} \}_{d=0}^D \\ \textit{such that } \sum_d a_d = t  }} \quad \prod_{d=0}^N \gamma_d^{a_d}
        \end{align}
        
        This class of optimality criteria can be seen as a generalization of the classical geometric discount. In fact, we highlight that for $D=0$, $\Phi_0(t) = \gamma_0^t$ which implies that $\mathcal{L}_0(\pi,r) = \mathcal{L}(\pi,r)$ for any policy $\pi$ and any reward function~$r$.
        In Figure~\ref{fig:coefficents}, we report the normalized distribution of the weights $\Phi_D(t)$ (i.e. $y(t) = \frac{\Phi_D(t)}{\sum_i \Phi_D(i)}$) over time as we vary the parameter $D \in \{0, \ldots, 9\}$. Notice how the mode of the probability distribution is shifted towards the right as we increased the delay, thus putting more weights on future time steps. 
        
        \begin{figure}[!ht]
            \centering
            \includegraphics[width=0.5\linewidth]{Figures/Coefficents.png}
            \caption{The normalized coefficients $\Phi_D(t)$ over time for different values of the delay parameter $D$}
             \label{fig:coefficents}
        \end{figure}
        % \begin{wrapfigure}[15]{r}{0.5\textwidth}
        %     \centering
        %     \includegraphics[width=0.5\textwidth]{Figures/Coefficents.png}
        %     \caption{\centering Cost weights over-time in $\mathcal{L}_D$}
        % \label{fig:coefficents}
        % \end{wrapfigure}
        
        % This new criterion $\mathcal{L}_D$ puts more weights on future time steps which reduces the bias against policies with longer mixing time. This can be observed in Figure \ref{fig:coefficents} where we reported the normalised distribution of the weights $\Phi_D(t)$ obtained by setting the discount factors to the value $\gamma_d=0.99$. As the depth $D$ increases, the mode of the probability distribution $\frac{\Phi_D(t)}{\sum_i \Phi_D(i)}$ is shifted toward the right, thus putting more weights on the future. 

        
        % In the following we discuss optimising linear combination of the introduced class of optimality criteria. Consider the following objective function: 
        % \begin{align*}
        %     \mathcal{L}_{\eta}(\pi, c) := \mathds{E}_{\pi, p_0}\Big[ \sum_t \eta(t) c_t \Big] \quad
        %     \textit{such that } \quad \eta(t) = \sum_{d=0}^D w_d \Phi_d(t)
        % \end{align*}
        % where the depth $D\in\mathds{N}$ and the coefficients $w_d\in\mathds{R}$ for any $d\in[0,D]$ are known. %The weights $\Phi_d(t)$ are also computed using some predefined discounts $\gamma_d\in(0,1)$ for any $d\in[0,D]$. 
        
        Intuitively, the proposed criterion ($\mathcal{L}_D$) describes the goal of an agent that discards short term gains in favor of long term discounted returns. In the following, we consider yet a more diverse problem formulation by using a linear combination of the delayed losses. Let $\mathcal{L}_\eta$ be the following objective function defined as: 
        \begin{align}
            \mathcal{L}_{\eta}(\pi, r) := \mathds{E}_{\pi, p_0}\Big[ \sum_t \eta(t) r_t \Big] \quad
            \textit{such that } \quad \eta(t) = \sum_{d=0}^D w_d \Phi_d(t)
        \end{align}
        where the depth $D\in\mathds{N}$ and the coefficients $w_d\in\mathds{R}$ for any $d\in[0,D]$ are known.
        
        In general, the optimal control in the sense of $\mathcal{L}_\eta$ is not stationary. However, learning solutions that admit compact representations is crucial for obvious computational reasons. 
        In the following we propose to learn either the optimal stationary solution, or to approximate the optimal control with a non-stationary policy over a finite horizon followed by a stationary one. 
        
        
    \subsection{Optimal stationary policies}
    \label{sec:optimal_stationary}
        In this section, we propose to learn stationary solution using a policy-iteration like algorithmic scheme. As in the classical setting, the goal is to learn a control $\pi^*$ that maximizes the state-action value function $Q_\eta^\pi$:
        
        \begin{align}
            Q_\eta^\pi(s,a) = \sum_{d=0}^D w_d Q_d^\pi(s,a) 
            \quad \textit{where} \quad 
            Q_d^\pi(s,a) := \mathds{E}_{\pi} \Big[ \sum_{t=0}^\infty \Phi_d(t) r_t | s_0,a_0=s,a\Big]
            \label{E:Q_eta_pi}
        \end{align}
        
        This is done by iteratively evaluating $Q_\eta^\pi$ and then updating the policy to maximize the learned value function. Due to the linearity illustrated in Equation \ref{E:Q_eta_pi}, the policy evaluation step is reduced to the estimation of $Q_d^\pi$. In geometrically discounted setting, the value function is the fixed point of the Bellman optimality operator. Luckily, this property is also valid for the quantities $Q_d^\pi$:
        
        \begin{proposition}
            For any discount parameters $(\gamma_d)_{d=0}^D$, the value functions $Q_D^\pi$ is the unique fixed point of the following $\gamma_D$-contraction:
            \begin{align}
                [T_{\pi}^D(q)](s,a) = \underbrace{ \mathds{E}_{\substack{s'\sim \mathcal{P}(s,a) \\ a'\sim\pi(s') }}\Big[r(s,a) + \sum_{d=0}^{D-1} \gamma_d Q_d^\pi(s',a') \Big] }_{\textstyle := r_D^\pi(s,a)} + \gamma_D \mathds{E}_{\substack{s'\sim \mathcal{P}(s,a) \\ a'\sim\pi(s') }} \Big[ q(s',a') \Big].
                \label{E:gamma_contraction}
            \end{align}
            \label{P:value_contraction}
        \end{proposition}
        The value $Q_D^\pi$ of a policy $\pi$ with respect to the delayed criterion $\mathcal{L}_D$ is the state-action value function of the same policy using an augmented policy dependent reward $r_D^\pi$ w.r.t. the $\gamma_D$-discounted returns. 
        Intuitively, the instantaneous worth of an action ($r_D^\pi$) is the sum of the environments' myopic returns ($r(s,a)$) and the long term evaluations (with lower delay parameters $(Q_d^\pi)_{d<D}$). 
        
        This has the beneficial side-effect of enhancing sample efficiency as it helps the agent to rapidly back-propagate long-term feed-backs to early states. 
        This reduces the time needed to distinguish good from bad behaviors, particularly in continuous settings where function approximation are typically used to learn policies.
        This is discussed in details in Section~\ref{sec:exp_continuous}.
        
        Similarly to standard value based RL algorithms, given a data set of trajectories $\mathcal{D}=\{s, a, s'\}$, the value function $Q_d^\pi$ can be approximated with parametric approximator $Q_{\theta_d}$ by optimising $J_d^Q(\theta)$: 
        \begin{align}
            J_D^Q(\theta) = \mathds{E}_{\substack{s,a,s' \sim \mathcal{D} \\ a' \sim \pi_\phi(s')}} \Big[ \frac{1}{2} \big( Q_\theta - ( r(s,a) + \sum_{d=0}^{D} \gamma_d Q_{\Bar{\theta}_d}(s',a'))^2  \big)  \Big]
            \label{E:value_function_loss}
        \end{align}
        As for the policy update step, inspired from the Soft-Actor-Critic (SAC) algorithm, we propose to optimize an entropy regularized soft Q-value using the following loss where $\alpha$ is a parameter:
        \begin{align}
            J_\eta^\pi(\phi) = -\mathds{E}_{s\sim\mathcal{D}, a\sim\pi_\phi}\Big[ \sum_{d=0}^D w_d Q_{\Bar{\theta}_d}(s,a) - \alpha\log(\pi_\phi(a|s)) \Big]
            \label{E:policy_loss}
        \end{align}
        
        We use Equations \ref{E:value_function_loss} and \ref{E:policy_loss} to construct Algorithm \ref{D-SAC}, a generalization of the SAC algorithm that approximates optimal stationary policies in the sense of $\mathcal{L}_\eta$. In practice, this can be further improved using the double Q-network trick and the automatic tuning of the regularization parameter $\alpha$. This is discussed in Appendix~\ref{supp:continuous_details}. Unfortunately, unlike the geometrically discounted setting, the policy improvement theorem is no longer guaranteed in the sense of $\mathcal{L}_\eta$. This means that depending on the initialization parameters, Algorithm $\ref{D-SAC}$ can either converge to the optimal stationary control or get stuck in a loop of sub-optimal policies. This is discussed in detail in Section \ref{sec:exp_hard_exp}.
        
        \begin{algorithm}[H]
            \caption{Generalized Soft Actor Critic}\label{D-SAC}
            \begin{algorithmic}[1]
                \STATE {\bfseries Input:} initial parameters $(\theta_d)_{d=0}^D, \phi$, learning rates $(\lambda_d)_{d=0}^D, \lambda_\pi$, pollyak parameter $\tau$
                \STATE initialise target network $\Bar{\theta}_d\leftarrow \theta_d$
                and initialise replay buffer $\mathcal{D}\leftarrow \emptyset$
                \FOR{each iteration}
                    \FOR{each environment step}
                        \STATE $a_t \sim \pi_\phi(s_t), \; s_{t+1} \sim \mathcal{P}(s_t,a_t), \; \mathcal{D} \leftarrow \mathcal{D} \cup \{ (s_t,a_t,s_{t+1},c_t) \}$
                    \ENDFOR
                    \FOR{$d \in [0, D]$}
                        \FOR{each $Q_d$ gradient step}
                            \STATE update parameter
                            $\theta_d \leftarrow \theta_d - \lambda_d \hat{\nabla}_{\theta_d}J_d^Q(\theta_d) $ 
                            and update target 
                            $ \Bar{\theta}_d \leftarrow \tau \Bar{\theta}_d + (1-\tau)\theta_d$
                        \ENDFOR
                    \ENDFOR
                    \FOR{each policy update}
                        \STATE update policy $\phi \leftarrow \phi - \lambda_\pi \hat{\nabla}_{\phi}J_\eta^\pi(\phi)$
                    \ENDFOR
                \ENDFOR
                \STATE {\bfseries Return:} $\pi_\phi, (Q_{\Bar{\theta}_d})_{d=0}^D$
            \end{algorithmic}
        \end{algorithm}
        
    \subsection{Approximate optimal control}
    \label{sec:optimal_control}
        In the general case, the optimal control is not necessarily stationary. Consider the problem of learning the optimal action profile $a_{0:\infty}^*$ which yields the following optimal value function: 
        \begin{align}
            V_\eta^*(s) := \max_{a_{0:\infty}}\mathds{E}_{a_{0:\infty}}\Big[\sum_{t=0}^\infty \eta(t) r_t | s_0=s\Big],
            \label{E:opt_control_value}
        \end{align}
        where $\mathds{E}_{a_{0:\infty}}$ is the expectation over trajectories generated using the designated action profile. 
        In this section we propose to solve this problem by approximating the value function from Equation \ref{E:opt_control_value}. This is achieved by applying the Bellman optimality principle in order to decompose $V_\eta^*$ into a finite horizon control problem (optimising $a_{0:H}$ with $H\in\mathds{N}$) and the optimal value function $V^*_{f^{H+1}(\eta)}$ where $f$ is an operator transforming the weighting distribution as follows: 
        \begin{align*}
            & \quad \Big[f(\eta)\Big](t) := \sum_{d=0}^D \big( \gamma_d \sum_{j=d}^D w_j \big) \Phi_d(t) = \langle\Gamma\cdot\Vec{w},\Vec{\Phi}(t)\rangle \\
            \textit{where } \quad & \Gamma := 
            \begin{bmatrix}
                \gamma_0 & \gamma_0 & \gamma_0 & ... & \gamma_0 \\
                0 & \gamma_1 & \gamma_1 & ... & \gamma_1 \\
                0 & 0 & \gamma_2 & ... & \gamma_2 \\
                \vdots & & & \ddots & \vdots \\
                0 & 0 & 0 & ... & \gamma_D 
            \end{bmatrix} \quad ; \quad
            \Vec{w}:= 
            \begin{bmatrix}
                w_0  \\
                w_1  \\
                w_2  \\
                \vdots \\
                w_D
            \end{bmatrix} \quad ; \quad
            \Vec{\Phi}(t):= 
            \begin{bmatrix}
                \Phi_0(t)  \\
                \Phi_1(t)  \\
                \Phi_2(t)  \\
                \vdots \\
                \Phi_D(t)
            \end{bmatrix} 
        \end{align*}
        For the sake of simplicity, let $\langle\Vec{1},\eta\rangle:=\sum_{d=0}^D w_d$ and $\big[f^n(\eta)\big](t):=\langle\Gamma^n\cdot\Vec{w},\Vec{\Phi}(t)\rangle$  for any $n,t\in\mathds{N}$.
        \begin{proposition}
            For any state $s_0\in\mathcal{S}$, the following identity holds: 
            \begin{align}
                V_\eta^*(s_0) = \max_{a_{0:H}} \Big\{ \mathds{E}_{a_{0:H}}\Big[\sum_{t=0}^H \langle\Vec{1},f^t(\eta)\rangle r_t\Big] + \mathds{E}_{a_0,a_1,..,a_{H}} \big[ V^*_{f^{H+1}(\eta)}(s_{H+1}) \big] \Big\}
                \label{bellman_general_H}
            \end{align}
            \label{P:bellman_general_H}
        \end{proposition}
        As a consequence, the optimal policy in the sense of $\mathcal{L}_\eta$ is to execute the minimising arguments $a_{0:H}^*$ of Equation \ref{bellman_general_H} and the execute the optimal policy in the sense $\mathcal{L}_{f^{H+1}(\eta)}$. Unfortunately, solving $\mathcal{L}_{f^{H+1}(\eta)}$ is not easier than the original problem. 
        
        However, under mild assumptions, for $H$ large enough, this criterion can be approximated with a simpler one. In order to derive this approximation, recall that the power iteration algorithm  described by the recurrence $\Vec{v}_{k+1}=\frac{\Gamma\cdot\Vec{v}_k}{\|\Gamma\cdot\Vec{v}_k\|}$ converges to the unit eigenvector corresponding to the largest eigenvalue of the matrix $\Gamma$ whenever that it is diagonalizable. In particular, if $0<\gamma_D<...<\gamma_0<1$ and $\Vec{v}_0=\Vec{w}$, then $\Gamma$ is diagonalizable, $\gamma_0$ is it's largest eigenvalue and the following holds:  
        \begin{align}
            \lim_{n\to\infty} \Vec{v}_{n+1} = \lim_{n\to\infty}\frac{\Gamma^n\cdot\Vec{w}}{\prod_{k\leq n}\|\Gamma\cdot\Vec{v}_k\|} = [\mathds{1}_{i=0}]_{i\in[0,D]} 
            \quad \textit{and} \quad \lim_{n\to\infty}\frac{V^*_{f^n(\eta)}(s)}{\prod_{k\leq n}\|\Gamma\cdot\Vec{v}_k\|} = V^*(s)
            \label{bellman_asymptotic}
        \end{align}
        Under these premises, the right hand term of the minimisation problem in Equation~\ref{bellman_general_H} can be approximated with the optimal value function in the sense of the classical RL criterion $\mathcal{L}$ (which optimal policy can be computed using any standard reinforcement learning algorithm in the literature). 
        
        Formally, we propose to approximate Equation \ref{bellman_general_H} with a proxy optimal value function $\Tilde{V}_{\eta, H}^*(s_0)$:
        \begin{align}
            \Tilde{V}_{\eta, H}^*(s_0) = \max_{a_{0:H}} \Big\{ \mathds{E}_{a_{0:H}}\Big[\sum_{t=0}^H \langle\Vec{1},f^t(\eta)\rangle r_t\Big] + \Big(\prod_{k\leq H}\|\Gamma\cdot\Vec{v}_k\|\Big) \mathds{E}_{a_0,a_1,..,a_{H}} \big[ V^*(s_{H+1}) \big] \Big\}
            \label{approx_bellman_general_H}
        \end{align}
        A direct consequence of Equation \ref{bellman_asymptotic} is that $\lim_{H\to\infty}\Tilde{V}_{\eta, H}^*(s)=V_\eta^*(s)$ for any state $s\in\mathcal{S}$. In addition, for a given horizon $H$, the optimal decisions in the sense of the proxy problem formulation are to execute for the first $H$ steps the minimising arguments $a_{0:H}^*$ of Equation \ref{approx_bellman_general_H} (they can be computed using dynamic programming) and then execute the optimal policy in the sense of the $\gamma_0$-discounted RL (which can be computed using any standard RL algorithm).
        
        \begin{algorithm}[ht]
            \caption{H-close optimal control}\label{H-OPT}
            \begin{algorithmic}[1]
                \STATE Compute $\pi^*, V^* \leftarrow \textsc{Policy Iteration}$ and initialize $\boldsymbol{v}_0\leftarrow\boldsymbol{w}$
                \FOR{$t\in[1,H]$}
                    \STATE Compute $\boldsymbol{v}_t\leftarrow \Gamma\cdot\boldsymbol{v}_{t-1} $
                \ENDFOR
                \STATE Initialise $\boldsymbol{V}_{H+1}(s) \leftarrow V^*(s) \cdot \prod_{k\leq H}\|\Gamma\cdot\Vec{v}_k\|$
                \FOR{$t\in[H,0]$}
                    \STATE Solve $\pi_t(s) \leftarrow \argmax_a \|\boldsymbol{v}_t\| \cdot c(s,a) + \mathds{E}_{s'\sim\mathcal{P}(s,a)}\big[ \boldsymbol{V}_{t+1}(s') \big]$
                    \STATE Compute $\boldsymbol{V}_t(s) \leftarrow \|\boldsymbol{v}_t\| \cdot c(s,\pi_t(s)) + \mathds{E}_{s'\sim\mathcal{P}(s,\pi_t(s))}\big[ \boldsymbol{V}_{t+1}(s') \big]$
                \ENDFOR
                \STATE {\bfseries Return:} $(\pi_t)_{t\in[0,H]}, \pi^*$
            \end{algorithmic}
        \end{algorithm}

==> (ICLR) RL with non geometric dicounts/Source/experiments.tex <==
\section{Experiments}
    \label{sec:experiments}
    In this section, we evaluate the performance of the proposed algorithm. Our goal is to answer the following questions: 
    \begin{itemize}
        \item How does the different parameters impact the ability of the proposed algorithms to solve hard exploration problems? 
        \item How does the proposed algorithm impact the performance in classical continuous control problems?
    \end{itemize}

    \subsection{Hard Exploration Problems}
    \label{sec:exp_hard_exp}
        In this section we investigate our ability to approximate the solution of the proposed family of RL problems (w.r.t. the optimality criterion $\mathcal{L}_D$) in discrete hard exploration maze environments. We fix the discount factor values to~\hbox{$\gamma_i = 0.99-\frac{i}{1000}$} throughout the experiments. This guarantees that $\Gamma$ is diagonalizable and that its largest eigenvalue is~\hbox{$\gamma_0=0.99$}.
        We evaluate the performance of both Algorithms \ref{D-SAC} and \ref{H-OPT} as we vary the depth parameter and as we increase the non stationarity horizon. 
        
        In Figure \ref{fig:env_rewards} we reported the shapes of the mazes as well as the used reinforcement signal in each of them. We used a sparse signal where the green dots represent the best achievable reward, the blue dots are associated with a deceptive reward and the red dots are associated with a penalty. This setting is akin to hard exploration problems as the agent might learn sub-optimal behaviour because of the deceiving signal or because of the penalty.
        \begin{figure}[ht]
             \centering
             \begin{subfigure}[b]{0.33\textwidth}
                 \centering
                 \includegraphics[width=\textwidth]{Figures/mazes/U_maze.png}
                 \caption{U-maze}
             \end{subfigure}
             \hfill
             \begin{subfigure}[b]{0.3\textwidth}
                 \centering
                 \includegraphics[width=\textwidth]{Figures/mazes/T_maze.png}
                 \caption{T-maze}
             \end{subfigure}
             \hfill
             \begin{subfigure}[b]{0.3\textwidth}
                 \centering
                 \includegraphics[width=\textwidth]{Figures/mazes/maze_0.png}
                 \caption{\centering Random maze}
             \end{subfigure}
            \caption{Hard exploration environments}
            \label{fig:env_rewards}
        \end{figure}
        
        \paragraph{Stationary solutions:} We start by evaluating the performances of the learned policies using Generalised Soft Actor Critic (GSAC) (Algorithm \ref{D-SAC}). As discussed earlier, unlike the geometrically discounted setting, the policy update is not guaranteed to improve the performances. For this reason, depending on the initialisation, the algorithm can either converge to the optimal stationary policy, or get stuck in a sequence of sub-optimal policies. 
        
        In Figure \ref{fig:discrete_optimal_stationnary}, we reported the performances of GSAC as we varied the depth hyper-parameter $D$ using two initialisation protocol. The blue curves are associated with a randomly selected initial parameters while the red curves are associated with experiment were the policy is initialised with the solution of the geometrically discounted problem. The solid lines correspond to the average reward while the dashed lines correspond to the $\Phi_d$ weighted loss (as computed in $\mathcal{L}_d$). 
        
        In all experiments, the expectations were averaged across $25$ runs of the algorithm using trajectories of length $4000$ initialised in all possible states (uniform $p_0$) . A common observation is that for a depth $D$ higher than 6~7 the algorithm was unstable and we couldn't learn a good stationary policy in a reliable way. However, the learned stationary policies with even a relatively shallow depth parameter yielded reliable policies that not only maximise the $\Phi_D$ weighted rewards but also improved the average returns. Notice how the baseline ($D=0$, i.e. the geometrically discounted case) always under-performs when compared to the learned policies for a depth parameter around 3.  
        
        We also observe that the algorithm is sensitive to the used initialisation. Using the optimal policy in the sens of the geometrically discounted objective (red curves) helped stabilise the learning procedure in most cases: this is particularly true in the random maze environment where a random initialisation of the policy yielded bad performances even with a low depth parameter. This heurestic is not guaranteed to produce better performances in all cases, notice how for $D=7$ in the T-maze, a random initialisation outperformed this heuristic consistently. 
        
        \begin{figure}[ht]
            \centering
            \includegraphics[width=\linewidth]{Figures/stationary_performances.png}
            \caption{Learned stationary policy (GSAC) performances as the depth parameter varies}
            \label{fig:discrete_optimal_stationnary}
        \end{figure}
        
        \paragraph{Optimal Control Approximation:}
        
        In this section we investigate the performances of the policies learned using Algorithm \ref{H-OPT} as we vary the non stationarity horizon $H$ for three depth parameters $D\in\{5,10,15\}$ (respectively the red, blue and green curves). As in the last experiment, we reported the expected returns as the average rewards using the continuous lines and as the $\Phi_D$ weighted rewards using dashed lines. As a baseline, we can observe in each figure the performances of the optimal policy in the sense of the geometrically discounted criterion when the non-stationarity horizon $H=0$. We also reported the performances of the best stationary policy learned using GSAC for a depth parameter $D=5$. 
        
        The first notable observation is that increasing the hyper-parameter $H$ does indeed improve performances. In addition, we notice that the maximum possible improvement is reached using a finite horizon $H$ (i.e. the maximising argument of both $\Tilde{V}_{\eta, H}$ and $V_\eta^*$ are the same). Intuitively, the $H$ non stationary steps enable the agent to get to an intermediate state from which the optimal policy in the sense of the discounted RL formulation can lead to the state with the highest rewards. This explains the effectiveness of current hard exploration RL algorithms\cite{ecoffet2019go,eysenbach2019search}: by learning a policy that reaches interesting intermediate state, these methods are implicitly learning an approximate solution of $\Tilde{V}_{\eta, H}$. 
        
        In the case of $D=5$, the obtained performances using Algorithm $\ref{H-OPT}$ converged to the performances of the optimal stationary policy obtained using GSAC in both the random and T-maze. On the other hand, unlike GSAC, the H-close algorithm is not sensitive to initialisation: in fact notice how even for arbitrarily high depth parameter ($D=15$) the learned policy ends up saturating the average and the $\Phi_D$ weighted rewards. More interestingly, increasing the depth can be beneficial as we observe empirically that for higher depth parameters, the non-stationarity horizon required to achieve the best possible performances decreases. 
        
        \begin{figure}[ht]
            \centering
            \includegraphics[width=\linewidth]{Figures/H_performances.png}
            \caption{Learned H-close optimal control}
            \label{fig:discrete_optimal_non_stationnary}
        \end{figure}
        
    
        %\begin{figure}[ht]
        %    \centering
        %    \includegraphics[width=\linewidth]{Figures/U_maze.png}
        %    \includegraphics[width=\linewidth]{Figures/T_maze.png}
        %    \includegraphics[width=\linewidth]{Figures/maze_0.png}
        %    \caption{Performances in hard exploration environments (U-maze, T-maze and random-maze)}
        %    \label{fig:optimal_non_stationnary}
        %\end{figure}
        
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \subsection{Simulated Continuous Control Benchmarks}
    \label{sec:exp_continuous}
    In this section, we propose to evaluate our methods on several continuous robotics domains. To this end, we consider 5 different environments within the \mujoco physics engine \citep{todorov2012mujoco}: Walker2d, Hopper, HalfCheetah, Ant and Humanoid. As results in the tabular settings showed that there exists a threshold beyond which increasing the value of the delay $D$ hurts the performance, we fix $D=1$, where only two discount factors $\gamma_0$ and $\gamma_1$ are used. We compare our proposed methods to the classic SAC algorithm to investigate the implications of using both critics $Q_{\theta_0}$ and $Q_{\theta_1}$.
    
    In Figure~\ref{fig:continuous_env_rewards}, we report the average rewards obtained by the different agents over time. Note that in all the environments, the GSAC agents are faster in collecting positive rewards than the SAC agents. The main reason behind this is that the critic tends to discern good from bad actions in the GSAC agents faster than the SAC agents. In fact, on the one hand, the SAC agents spend more time uncertain about the quality of their actions for a given state, and thus need more time and more experience to make the estimations of their critic more accurate and reflecting the true long-term value of an action. On the other hand, in the GSAC agents, $Q_{\theta_1}$ takes into consideration the estimate of the actions by $Q_{\theta_0}$, and thus there is less uncertainty about their quality. 
    
    
    \begin{figure}[ht]
             \centering
             \begin{subfigure}[b]{0.4\textwidth}
                 \centering
                 \includegraphics[width=\textwidth]{Figures/continuous/Walker2d-v2_1.pdf}
             \end{subfigure}
             \begin{subfigure}[b]{0.4\textwidth}
                 \centering
                 \includegraphics[width=\textwidth]{Figures/continuous/Hopper-v2_sr_compressed.pdf}
             \end{subfigure}\\
             \begin{subfigure}[b]{0.4\textwidth}
                 \centering
                 \includegraphics[width=\textwidth]{Figures/continuous/HalfCheetah-v2_sr_compressed.pdf}
             \end{subfigure}
             \begin{subfigure}[b]{0.4\textwidth}
                 \centering
                 \includegraphics[width=\textwidth]{Figures/continuous/Ant-v2_sr_compressed.pdf}
             \end{subfigure}
            \caption{\centering Training curves on continuous control benchmarks. Generalized Soft-Actor-Critic (GSAC) shows better sample efficiency across all tasks}
            \label{fig:continuous_env_rewards}
        \end{figure}

==> (ICLR) RL with non geometric dicounts/Source/family_problems.tex <==
\section{Beyond the geometric discount}
    In order to reduce the bias against policies with longer mixing times without having to deal with numerical instabilities (by choosing a high discount factor) nor requiring a particular MDP structure (in order to explicitly solve the average cost formulation), we propose to solve the RL problem using a more flexible weighting distribution. 
    
    \subsection{A particular family of optimality criterion}
        For a given depth parameter $D\in\mathbb{N}$, we define the discount factors $\gamma_d \in(0,1)$ for any integer $d\in[0,D]$ and we consider the following optimality criterion:
        \begin{align}
            \mathcal{L}_D(\pi, c) := \mathbb{E}_{\pi, p_0} \Big[ \sum_{t=0}^\infty \Phi_D(t) c_t \Big] 
            \quad \textit{where} \quad 
            \Phi_D(t) := \sum_{\substack{ \{a_d \in \mathbb{N} \}_{i=0}^N \\ \textit{such that } \sum_d a_d = t  }} \quad \prod_{d=0}^N \gamma_d^{a_d}
        \end{align}
        
        
        \begin{wrapfigure}[15]{r}{0.5\textwidth}
            %\centering
            \includegraphics[width=0.5\textwidth]{Figures/Coefficents.png}
            \caption{\centering Cost weights over-time in $\mathcal{L}_D$}
        \label{fig:coefficents}
        \end{wrapfigure}
        
        This new criterion $\mathcal{L}_D$ puts more weights on future time steps which reduces the bias against policies with longer mixing time. This can be observed in Figure \ref{fig:coefficents} where we reported the normalised distribution of the weights $\Phi_D(t)$ obtained by setting the discount factors to the value $\gamma_d=0.99$. In fact, as $N$ increases, the mode of the probability distribution $\frac{\Phi_D(t)}{\sum_i \Phi_D(i)}$ is shifted toward the right, thus putting more weights on the future. 
        
        In addition, this class of optimality criterions can be seen as a generalisation of the classical geometric discount. In fact, we highlight that $\Phi_0(t) = \gamma_0^t$ which implies that $\mathcal{L}_0(\pi,c) = \mathcal{L}(\pi,c)$ for any policy $\pi$ and any cost function~$c$.
        
        In order to optimise this new criterion, we define the associated value functions:
        \begin{align*}
            V_D^\pi(s) := \mathbb{E}_{\pi} \Big[ \sum_{t=0}^\infty \Phi_D(t) c_t | s_0=s\Big] \; ; \;
            Q_D^\pi(s,a) := \mathbb{E}_{\pi} \Big[ \sum_{t=0}^\infty \Phi_D(t) c_t | s_0,a_0=s,a\Big]
        \end{align*}
        Similarly to the case of geometrically discounted RL (i.e. $D=0$), the obtained values functions are the fixed point of a particular operator that we derive in the following section.
        
    \subsection{Value functions are the unique fixed point of a Bellman like operator}
        To derive the desired operator, it is useful to derive a relationship between the coefficients~$\Phi_D(t)$: 
        \begin{Lemma}
            For any integer $D>0$ , the following equalities hold: 
            \begin{align*}
                \Phi_D(t) = \sum_{k=0}^t \gamma_D^k \Phi_{D-1}(t-k) = \Phi_{D-1}(t) + \gamma_D \Phi_D(t-1) = \sum_{d=0}^D \gamma_d \Phi_d(t-1)
            \end{align*}
            \label{L:weight_property}
        \end{Lemma}
        
        The latter equality in the previous lemma expresses the weight of the $t^\textit{th}$ cost in $\mathcal{L}_D$ as a linear combination of the weights of the previous time stamp ($t-1$) in $\mathcal{L}_{d}$ for $d\leq D$. This is used to establish the following relationship between the value functions $V_D^\pi(s)$ for any state $s\in\mathcal{S}$:
        \begin{proposition}
            For any state $s\in\mathcal{S}$ and for any integer $D\in\mathbb{N}$, we have:
            \begin{align*}
                V_D^\pi(s) = \mathbb{E}_{\substack{a\sim\pi(s) \\ s'\sim \mathcal{P}(s,a) }} \Big[c(s,a) + \sum_{d=0}^D \gamma_d V_d^\pi(s') \Big] 
            \end{align*}
            \label{P:value_decomposition}
        \end{proposition}
        Notably we can re-write the latter equality as: 
        \begin{align}
            V_D^\pi(s) = \underbrace{ \mathbb{E}_{\substack{a\sim\pi(s) \\ s'\sim \mathcal{P}(s,a) }} \Big[c(s,a) + \sum_{d=0}^{D-1} \gamma_d V_d^\pi(s') \Big]}_{\textstyle := c_D(s,a) } + \gamma_D \mathbb{E}_{\substack{a\sim\pi(s) \\ s'\sim \mathcal{P}(s,a) }} \Big[V_D^\pi(s')\Big]
            \label{bellman_V_d}
        \end{align}
        where $c_D(s,a)$ is an augmented cost function entirely defined through the MDP's cost function $c$ and the value functions $V_d^\pi$ for $d<D$. It ensues from this derivation that the value function $V_D^\pi$ is the unique fixed point of the following $\gamma_D$-contraction:
        \begin{align*}
            [T_{\pi}^D(v)](s) = \mathbb{E}_{\substack{a\sim\pi(s) \\ s'\sim \mathcal{P}(s,a) }} \Big[c_D(s,a) + \gamma_D v(s') \Big].
        \end{align*}
        A practical implication of this property is a tractable algorithmic approach to compute $V_D^\pi$ using any classical policy evaluation technique:
        \begin{algorithm}
            \caption{D-deep policy evaluation}\label{D-PE}
            \begin{algorithmic}[1]
                \STATE {\bfseries Input:} Depth parameter $D$, the cost function $c_0=c$, the policy $\pi$, the dynamics $\mathcal{P}$ (or \hbox{$\pi$-generated trajectories}), and a policy evaluation algorithm
                \FOR{$d \in [0, D]$}
                \STATE Evaluate $V_d^\pi$ using policy evaluation and the cost $c_d$ 
                \STATE Learn the cost $c_d(s,a) = \mathbb{E}_{\substack{a\sim\pi(s) \\ s'\sim \mathcal{P}(s,a) }} \Big[ c(s,a) + \sum_{i=0}^{d} \gamma_i V_i^\pi(s') \Big]$
                \ENDFOR
                \STATE {\bfseries Return:} $V_D^\pi$
            \end{algorithmic}
        \end{algorithm}
        Naturally, the latter algorithm can solve the problem exactly in tabular settings if the transition dynamics are provided. In more complex settings (continuous state/action space, unknown dynamics), sample-based policy evaluation techniques can be used to evaluate the third step and a supervised learning algorithm can be used to solve the fourth step. 
        
        We also point out that a similar reasoning can be applied to evaluate the Q-function associated to the $\mathcal{L}_D$ criterion. In fact, using Equation \eqref{bellman_V_d}, the following equality holds:
        \begin{align*}
            Q_D^\pi(s,a) = c(s,a) + \mathbb{E}_{s'\sim \mathcal{P}(s,a)}\Big[\sum_{d=0}^{D-1} \gamma_d V_d^\pi(s') \Big] + \gamma_D \mathbb{E}_{\substack{s'\sim \mathcal{P}(s,a) \\ a' \sim \pi(s')}}\Big[Q_D^\pi(s',a') \Big]
        \end{align*}
        
        This implies that $Q_D^\pi$ is also the unique fixed point of a $\gamma_D$-contraction. Practically it can be estimated with a similar scheme to the one presented in Algorithm \ref{D-PE}.
      

==> (ICLR) RL with non geometric dicounts/Source/optimal_planning.tex <==
\section{General non-geometrically discounted optimal decision making}
    In this section we discuss optimising a more general class of optimality criteria. Consider the following objective function: 
    \begin{align*}
        \mathcal{L}_{\eta}(\pi, c) := \mathbb{E}_{\pi, p_0}\Big[ \sum_t \eta(t) c_t \Big] \quad
        \textit{such that } \quad \eta(t) = \sum_{d=0}^D w_d \Phi_d(t)
    \end{align*}
    where the depth $D\in\mathbb{N}$ and the coefficients $w_d\in\mathbb{R}$ for any $d\in[0,D]$ are known. The weights $\Phi_d(t)$ are also computed using some predefined discounts $\gamma_d\in(0,1)$ for any $d\in[0,D]$. 
    
    This class of optimality criteria encapsulates in particular the geometrically discounted objective function. In fact setting $\eta = \Phi_0$ entails that $\mathcal{L}_\eta=\mathcal{L}_0=\mathcal{L}$.
    
    In this section, our goal is to provide a tractable approach to approximate the optimal sequence of actions that optimises $\mathcal{L}_\eta$. For this reason, we define the optimal value function as:
    \begin{align*}
        V_\eta^*(s) := \min_{a_{0:\infty}}\mathbb{E}_{a_{0:\infty}}\Big[\sum_{t=0}^\infty \eta(t) c_t | s_0=s\Big] \; ; \; Q_\eta^*(s,a) := \min_{a_{1:\infty}}\mathbb{E}_{a_{1:\infty}}\Big[\sum_{t=0}^\infty \eta(t) c_t | s_0,a_0=s,a\Big]
        %V_\eta^\pi(s) := \mathbb{E}_{\pi} \Big[ \sum_{t=0}^\infty \eta(t) c_t | s_0=s\Big] 
        %\; ; \; 
        %Q_\eta^\pi(s,a) := \mathbb{E}_{\pi} \Big[ \sum_{t=0}^\infty \eta(t) c_t | s_0,a_0=s,a\Big] 
    \end{align*}
    Where $\mathbb{E}_{a_0, a_1, ...}$ is the expectation over trajectories generated using the designated action profile. 
      
    \subsection{Optimal stationary policy}
        Given a stationary policy $\pi$, the associated value function in the sense of $\mathcal{L}_\eta$ can be decomposed into: 
        \begin{align}
            V_\eta^\pi(s) = \sum_{d=0}^D w_d V_d^\pi(s) \quad ; \quad Q_\eta^\pi(s,a) = \sum_{d=0}^D w_d Q_d^\pi(s,a)
            \label{value_linear_decomp}
        \end{align}
    
        In general, there is no guarantee that the optimal policy is stationary. However, the optimal stationary policy $\pi^*$ in the sense of $\mathcal{L}_\eta$ verifies $\pi^*(s) \in  \argmin_{a} Q_\eta^{\pi^*}(s,a)$ for any state $s\in \mathcal{S}$. For this reason, and similarly to policy evaluation algorithm, we propose to approximate the solution using the following two step procedure:
        \begin{itemize}
            \item \textbf{Policy evaluation step:} Evaluate $Q_\eta^{\pi_k}$ using deep-policy evaluation and Equation \eqref{value_linear_decomp}
            \item \textbf{Policy \st{improvement} update step:} Update the policy: $\pi_{k+1}(s)=\argmax_a Q_\eta^{\pi_k}(s,a)$
        \end{itemize}
        Unfortunately, the policy improvement theorem is no longer valid in this setting. For this reason, the proposed update rule does not guarantee a systematic improvement over the iterations. In practice, we noticed that the algorithm either converges to the optimal stationary policy, or gets stuck in a loop. 
        
        
    \subsection{Optimal decision making}
        The bellman optimality principle in this setting can be used to derive a relationship between $V_\eta^*$ and $V_{f(\eta)}^*$ where $f$ is an operator transforming the weighting distribution as follows: 
        \begin{align*}
            & \quad \Big[f(\eta)\Big](t) := \sum_{d=0}^D \big( \gamma_d \sum_{j=d}^D w_j \big) \Phi_d(t) = \langle\Gamma\cdot\Vec{w},\Vec{\Phi}(t)\rangle \\
            \textit{where } \quad & \Gamma := 
            \begin{bmatrix}
                \gamma_0 & \gamma_0 & \gamma_0 & ... & \gamma_0 \\
                0 & \gamma_1 & \gamma_1 & ... & \gamma_1 \\
                0 & 0 & \gamma_2 & ... & \gamma_2 \\
                \vdots & & & \ddots & \vdots \\
                0 & 0 & 0 & ... & \gamma_D 
            \end{bmatrix} \quad ; \quad
            \Vec{w}:= 
            \begin{bmatrix}
                w_0  \\
                w_1  \\
                w_2  \\
                \vdots \\
                w_D
            \end{bmatrix} \quad ; \quad
            \Vec{\Phi}(t):= 
            \begin{bmatrix}
                \Phi_0(t)  \\
                \Phi_1(t)  \\
                \Phi_2(t)  \\
                \vdots \\
                \Phi_D(t)
            \end{bmatrix} 
        \end{align*}
        The following proposition introduces the underlying relationship formally: 
        \begin{proposition}
            For any state $s_0\in\mathcal{S}$, the following identity holds: 
            \begin{align}
                V_\eta^*(s_0) = \min_{a_0} \Big\{ \big[\sum_{d=0}^D w_d\big] c(s_0,a_0) + \mathbb{E}_{s_1} \big[ V^*_{f(\eta)}(s_1) \big] \Big\}
                \label{bellman_general}
            \end{align}
            \label{P:bellman_general}
        \end{proposition}
        For the sake of simpler notations, let $\langle\Vec{1},\eta\rangle:=\sum_{d=0}^D w_d$ and let $\big[f^n(\eta)\big](t):=\langle\Gamma^n\cdot\Vec{w},\Vec{\Phi}(t)\rangle$  for any $n,t\in\mathbb{N}$. Using Equation \eqref{bellman_general} and an inductive reasoning w.r.t the horizon $H\in\mathbb{N}$ we get: 
        \begin{align}
            V_\eta^*(s_0) = \min_{a_{0:H}} \Big\{ \mathbb{E}_{a_{0:H}}\Big[\sum_{t=0}^H \langle\Vec{1},f^t(\eta)\rangle c_t\Big] + \mathbb{E}_{a_0,a_1,..,a_{H}} \big[ V^*_{f^{H+1}(\eta)}(s_{H+1}) \big] \Big\}
            \label{bellman_general_H}
        \end{align}
        As a consequence, the optimal policy in the sense of $\mathcal{L}_\eta$ is to execute the minimising arguments $a_{0:H}^*$ of Equation \eqref{bellman_general_H} and the execute the optimal policy in the sense $\mathcal{L}_{f^{H+1}(\eta)}$. Unfortunately, solving $\mathcal{L}_{f^{H+1}(\eta)}$ is not easier than the original problem. 
        
        However, under mild assumptions, for $H$ large enough, this criterion can be approximated with a simpler one. In order to derive this approximation, recall that the power iteration algorithm  described by the recurrence $\Vec{v}_{k+1}=\frac{\Gamma\cdot\Vec{v}_k}{\|\Gamma\cdot\Vec{v}_k\|}$ converges to the unit eigenvector corresponding to the largest eigenvalue of the matrix $\Gamma$ whenever that it is diagonalizable. In particular, if $0<\gamma_D<...<\gamma_0<1$ and $\Vec{v}_0=\Vec{w}$, then $\Gamma$ is diagonalizable, $\gamma_0$ is it's largest eigenvalue and the following holds:  
        \begin{align}
            \lim_{n\to\infty} \Vec{v}_{n+1} = \lim_{n\to\infty}\frac{\Gamma^n\cdot\Vec{w}}{\prod_{k\leq n}\|\Gamma\cdot\Vec{v}_k\|} = [\mathbb{1}_{i=0}]_{i\in[0,D]} 
            \quad \textit{and} \quad \lim_{n\to\infty}\frac{V^*_{f^n(\eta)}(s)}{\prod_{k\leq n}\|\Gamma\cdot\Vec{v}_k\|} = V^*(s)
            \label{bellman_asymptotic}
        \end{align}
        Under these premises, the right hand term of the minimisation problem in Equation~\eqref{bellman_general_H} can be approximated with the optimal value function in the sense of the classical RL criterion $\mathcal{L}$ (which optimal policy can be computed using any standard reinforcement learning algorithm in the literature). 
        
        Formally, we propose to approximate Equation \eqref{bellman_general_H} with a proxy optimal value function $\Tilde{V}_{\eta, H}^*(s_0)$:
        \begin{align}
            \Tilde{V}_{\eta, H}^*(s_0) = \min_{a_{0:H}} \Big\{ \mathbb{E}_{a_{0:H}}\Big[\sum_{t=0}^H \langle\Vec{1},f^t(\eta)\rangle c_t\Big] + \Big(\prod_{k\leq H}\|\Gamma\cdot\Vec{v}_k\|\Big) \mathbb{E}_{a_0,a_1,..,a_{H}} \big[ V^*(s_{H+1}) \big] \Big\}
            \label{approx_bellman_general_H}
        \end{align}
        A direct consequence of Equation \ref{bellman_asymptotic} is that $\lim_{H\to\infty}\Tilde{V}_{\eta, H}^*(s)=V_\eta^*(s)$ for any state $s\in\mathcal{S}$. In addition, for a given horizon $H$, the optimal decisions in the sense of the proxy problem formulation are to execute for the first $H$ steps the minimising arguments $a_{0:H}^*$ of Equation \eqref{approx_bellman_general_H} (they can be computed using dynamic programming) and then execute the optimal policy in the sense of the $\gamma_0$-discounted RL (which can be computed using any standard RL algorithm).
        

==> (ICLR) RL with non geometric dicounts/Source/related.tex <==
\section{Related Work}

\paragraph{Bridging the gap between discounted and average rewards criteria. }
    % bias against policies with longer mixing times 
    % average reward formulation
    % learning behaviours over different time scale
    % blackwell opt
    % numerical instabilities + \gamma related approaches
    
    It is well known that defining optimality with respect to the cumulative discounted reward criterion induces a built-in bias against policies with longer mixing times. In fact, due to the exponential decay of future returns, the contribution of the behaviour from the $T^{\textit{th}}$ observation up to infinity is scaled down by a factor of the order of $\gamma^T$. In the literature, the standard approach to avoid this downfall is to define optimality with respect to the average reward criterion $\Bar{\mathcal{L}}$ defined as : 
    \begin{align*}
        \Bar{\mathcal{L}}(\pi,r) := \lim_{T\to\infty} \frac{1}{T} \mathds{E}_{\pi, p_0}\Big[ \sum_{t=0}^T r_t \Big] 
    \end{align*}
    This setting as well as dynamic programming algorithms for finding the optimal average return policies have been long studied in the literature \citep{howard1960dynamic, veinott1966finding, blackwell1962discrete, puterman2014markov}. Several value based approaches \citep{schwartz1993reinforcement, abounadi2001learning, wei2020model} as well as policy based ones \citep{kakade2001optimizing, baxter2001infinite} have been investigated to solve this problem. These approaches are limited in the sense that they require particular MDP structures to enjoy theoretical guarantees. 
    
    % multiple geometrically discounted objective
    % learning the value function for different discounts
    % using hyperbolic discounts
    
    %Alternatively, RL researchers investigated formulations beyond the fixed discount model to alleviate the time-scale dependency of the learned policy. 
    %For example, it is possible to optimise $\gamma$-discounted returns under some constraint over a similar objective with a different discount factor. 
    %Or to learn the value function across different discounts values to induce an improved predictive power across a wider range of discounts
    
    Another line of research, is based on the existence of a critical discount factor $\gamma_{\textit{crit}}<1$ such that for any discount $\gamma\in(\gamma_{\textit{crit}},1)$ the optimal policy in the sense of the $\gamma$-discounted criterion also optimises the average returns \cite{blackwell1962discrete}. Unfortunately, this critical value can be arbitrarily close~to~$1$ which induces computational instabilities in practice. For this reason, previous works attempted to mitigate this issue by increasing the discount factor during training \citep{prokhorov1997adaptive}, learning higher-discount solution via learning a sequence of lower-discount value functions \citep{romoff2019separating} or tweaking the reinforcement signal to equivalently learn the optimal policy using lower discounts \citep{tessler2020reward}.


\paragraph{Exploration Strategies. }
    Another line of research attempted to tackle the hard exploration problem by further driving the agents exploration towards interesting states. 
    % Intrinsic motivation based exploration
    Inspired by intrinsic motivation in psychology \citep{oudeyer2008can}, some approaches train policies with rewards composed of extrinsic and intrinsic terms. Namely, count-based exploration methods keep track of the agents' past experience and aim at guiding them towards rarely visited states rather than common ones \citep{bellemare2016unifying, colas2019curious}. Alternatively, prediction-based exploration define the intrinsic rewards with respect to the agents' familiarity with their environments by estimating a dynamics prediction model \citep{stadie2015incentivizing, pathak2019self}.
    % Memory-based Exploration
    Other approaches maintain a memory of interesting states \citep{ecoffet2019go, ecoffet2021first}, trajectories \citep{guo2019memory} or goals \citep{guo2019directed}. \citet{ecoffet2019go, ecoffet2021first} first return to interesting states using either a deterministic simulator or a goal-conditioned policy and start exploration from there. \citep{guo2019memory} train a trajectory-based policy to rather prefer trajectories that end with rare states. \citet{guo2019directed} revisit goals that have higher uncertainty. 
    % Options based Exploration
    Finally, based on the options framework \citep{sutton1999between}, options-based exploration aims at learning policies with termination conditions—or macro-actions. This allows the introduction of abstract actions, hence driving the agents' exploration towards behaviours of interest \citep{gregor2016variational, achiam2017variational}.
    
    
    


==> (ICLR) RL with non geometric dicounts/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> (ICLR) RL with non geometric dicounts/preamble.tex <==
\usepackage{hyperref}
\usepackage{ucs}
\usepackage{comment}
\usepackage{amsmath}
\usepackage{bbold}
%\usepackage{fancybox}%fait des boites
\usepackage{pbox}%fait des boites
\usepackage{tcolorbox}
\usepackage[font=small]{caption}
\usepackage{capt-of}
%\usepackage{subcaption} % incompatible with subfig
%\usepackage[numbers]{natbib}
\usepackage{bm}
\usepackage{graphicx}
\usepackage{cancel}
\usepackage{array}
\usepackage{multirow}
\usepackage{colortbl}
\usepackage{tikz}
\usepackage{xspace}
\usepackage{algorithm}
\usepackage[noend]{algorithmic}
% \usepackage[noend]{algpseudocode}
\usepackage{soul}
\usepackage{enumitem}
\usepackage{comment}
\usepackage{wrapfig}
% \usepackage[caption=false,font=footnotesize]{subfig}
\usepackage{subcaption}
%\usepackage{apalike}
%\usepackage{cite}
\usepackage{dsfont}

%\renewcommand{\cite}{\citep}

\newcommand{\dhh}{\mymath{dh}}
\newcommand{\vth}{\mymath{\vec \theta}}
\newcommand{\vthp}{\mymath{\vec \vth^\prime}}
\newcommand{\delth}{\mymath{\delta \vth}}
\newcommand{\delthp}{\mymath{\delta \vthp}}
\newcommand{\hth}{\mymath{h_{\vth}}}
\newcommand{\hdth}{\mymath{h_{\vth + \delth}}}
\newcommand{\grad}{\mymath{\nabla_{\vth}}}
\newcommand{\natgrad}{\mymath{\nabla^{nat}_{\vth}}}
\newcommand{\Mnat}{\mymath{\vec M_{\text{nat}}(\vth)}}
\newcommand{\Hess}{\mymath{\vec H(\vth)}}
\newcommand{\C}{\mymath{\bf C(\vth)}}
\newcommand{\kfac}{{\sc kfac}\xspace}
\newcommand{\cemrl}{{\sc cem-rl}\xspace}
\newcommand{\cemddpg}{{\sc cem-ddpg}\xspace}
\newcommand{\cemtdd}{{\sc cem-td3}\xspace}
\newcommand{\relu}{{\sc relu}\xspace}
\newcommand{\evorl}{{\sc erl}\xspace}
\newcommand{\hc}{{\sc half-cheetah-v2}\xspace}
\newcommand{\hop}{{\sc hopper-v2}\xspace}
\newcommand{\sw}{{\sc swimmer-v2}\xspace}
\newcommand{\ant}{{\sc ant-v2}\xspace}
\newcommand{\walk}{{\sc walker2d-v2}\xspace}
\newcommand{\muj}{{\sc mujoco}\xspace}
\newcommand{\geppg}{{\sc gep-pg}\xspace}
\newcommand{\pytorch}{{\sc PyTorch}\xspace}

\newcommand{\mdp}{{\sc mdp}\xspace}
\newcommand{\gamer}{{\sc gamer}\xspace}
\newcommand{\gargaml}{{\sc gargaml}\xspace}
\newcommand{\tddd}{{\sc td3}\xspace}

\newcommand{\gnn}{{\sc gnn}\xspace}
\newcommand{\gnns}{{\sc gnn}s\xspace}
\newcommand{\cnn}{{\sc cnn}\xspace}
\newcommand{\cnns}{{\sc cnn}s\xspace}
\newcommand{\gorl}{{\sc gorl}\xspace}
\newcommand{\imrl}{{\sc imrl}\xspace}
\newcommand{\nl}{{\sc nl}\xspace}

%%% Math commands
\def\bbbr{{\rm I\!R}}
\def\bbbe{{\rm I\!E}}
% \newcommand{\R}{{\bbbr}{}}
\newcommand{\Esp}{{\bbbe}{}}
\renewcommand\Pr{P} % probability
\newcommand\esper[2]{\underset{#1}{\mathbb{E}} \left[#2\right]} % expectation
\newcommand\espernosubstack[2]{\mathbb{E}_{#1} \left[#2\right]} % expectation, without substacking #1
\newcommand\espernobr[1]{\underset{#1}{\mathbb{E}}} % expectation, without brackets
\newcommand\mymax[2]{\textmd{max}_{#1} ~ #2} % max
% \newcommand\argmin[2]{\textmd{argmin}_{#1} ~ #2} % argmin
\newcommand\trace{\textmd{Tr}} % trace operator
\newcommand\erf{\textmd{erf}} % error function
\newcommand\diag{\textmd{diag}} % diagonal matrix
\newcommand\asinh{\textmd{asinh}} % arcsinh
% \newcommand\KL[2]{D_{KL}\left(#1\|#2\right)} % Kullback-Leibler divergence
\newcommand\Id{\mat{I}}% identity matrix
\newcommand{\rbd}{{\sc rbd}\xspace}
\newcommand{\rbfn}{{\sc rbfn}\xspace}
\newcommand{\rbfns}{{\sc rbfn}s\xspace}
\newcommand{\vips}{{\sc vips}\xspace}
\newcommand{\reps}{{\sc reps}\xspace}
\newcommand{\creps}{{\sc creps}\xspace}
\newcommand{\hireps}{{\sc hireps}\xspace}
\newcommand{\aaac}{{\sc a3c}\xspace}
\newcommand{\offpac}{{\sc offpac}\xspace}
\newcommand{\reinforce}{{\sc reinforce}\xspace}
\newcommand{\retrace}{{\sc retrace}\xspace}
\newcommand{\blackdrops}{{\sc black-DROPS}\xspace}
\newcommand{\rock}{{\sc rock}$^*$\xspace}
\newcommand{\ddpg}{{\sc ddpg}\xspace}
\newcommand{\naf}{{\sc naf}\xspace}
\newcommand{\qprop}{{\sc Q-prop}\xspace}
\newcommand{\acer}{{\sc acer}\xspace}
\newcommand{\pgql}{{\sc pgql}\xspace}
\newcommand{\ipg}{{\sc ipg}\xspace}
\newcommand{\cmaes}{{\sc cma-es}\xspace}
\newcommand{\cma}{{\sc cma}\xspace}
\newcommand{\nes}{{\sc nes}\xspace}
\newcommand{\xnes}{x{\sc nes}\xspace}
\newcommand{\pepg}{{\sc pepg}\xspace}
\newcommand{\rwr}{{\sc rwr}\xspace}
\newcommand{\crkr}{{\sc crkr}\xspace}
\newcommand{\gpomdp}{{\sc g(po)mdp}\xspace}
\newcommand\cems{\textsc{cem}s\xspace}
\newcommand\cem{\textsc{cem}\xspace}
\newcommand{\trpo}{{\sc trpo}\xspace}
\newcommand{\ppo}{{\sc ppo}\xspace}
\newcommand{\gps}{{\sc gps}\xspace}
\newcommand{\nac}{{\sc nac}\xspace}
\newcommand{\enac}{e{\sc nac}\xspace}
\newcommand{\inac}{i{\sc nac}\xspace}
\newcommand{\sac}{{\sc sac}\xspace}
\newcommand{\acktr}{{\sc acktr}\xspace}
\newcommand{\ilqg}{i{\sc lqg}\xspace}
\newcommand{\svg}{{\sc svg}\xspace}
\newcommand{\power}{{\sc PoWER}\xspace}
\newcommand{\pilco}{{\sc pilco}\xspace}
\newcommand{\PIBB}{{\sc pi$^{\mbox{\tiny BB}}$}\xspace}
\newcommand{\picma}{{\sc pi$^2$-cma}\xspace}
\newcommand{\pis}{{\sc pi$^{2}$}\xspace}
\newcommand{\ann}{{\sc ann}\xspace}
\newcommand{\anns}{{\sc ann}s\xspace}
\newcommand{\mlps}{{\sc mlp}s\xspace}
\newcommand{\mlp}{{\sc mlp}\xspace}
\newcommand{\rbf}{{\sc rbf}\xspace}
\newcommand{\lwpr}{{\sc lwpr}\xspace}
\newcommand{\nipals}{{\sc nipals}\xspace}
\newcommand{\cad}{{\sc cad}\xspace}
\newcommand{\lcs}{{\sc lcs}\xspace}
\newcommand{\lcss}{{\sc lcs}s\xspace}
\newcommand{\xcsf}{{\sc xcsf}\xspace}
\newcommand{\QR}{{\sc qr}\xspace}
\newcommand{\RR}{{\sc rr}\xspace}
\newcommand{\xcs}{{\sc xcs}\xspace}
\newcommand{\moe}{{\sc m}o{\sc e}\xspace}
\newcommand{\gmr}{{\sc gmr}\xspace}
\newcommand{\gmm}{{\sc gmm}\xspace}
\newcommand{\gmms}{{\sc gmm}s\xspace}
\newcommand{\dmps}{{\sc dmp}s\xspace}
\newcommand{\mdps}{MDPs\xspace}
\newcommand{\ilogmr}{{\sc ilo-gmr}\xspace}
\newcommand{\kdtrees}{{\em kd-trees}\xspace}
\newcommand{\libsvm}{{\sc libsvm}\xspace}
\newcommand{\svd}{{\sc svd}\xspace}
\newcommand{\rmrc}{{\sc rmrc}\xspace}
\newcommand{\nmse}{{\sc nmse}\xspace}
\newcommand{\nmae}{{\sc nmae}\xspace}
\newcommand{\imlm}{{\sc imlm}\xspace}
\newcommand{\mae}{{\sc mae}\xspace}
\newcommand{\ga}{{\sc ga}\xspace}
\newcommand{\pls}{{\sc pls}\xspace}
\newcommand{\ls}{{\sc ls}\xspace}
\newcommand{\rlearning}{{\sc rl}\xspace}
\newcommand{\drl}{deep RL\xspace}
\newcommand{\Drl}{Deep RL\xspace}
\newcommand{\dqn}{{\sc dqn}\xspace}
\newcommand{\rls}{{\sc rls}\xspace}
\newcommand{\krls}{{\sc krls}\xspace}
\newcommand{\rfrls}{{\sc rfrls}\xspace}
\newcommand{\irfrls}{i{\sc rfrls}\xspace}
\newcommand{\issgpr}{i{\sc ssgpr}\xspace}
\newcommand{\rgls}{{\sc rgls}\xspace}
\newcommand{\krgls}{{\sc krgls}\xspace}
\newcommand{\lwr}{{\sc lwr}\xspace}
\newcommand{\lwpls}{{\sc lwpls}\xspace}
\newcommand{\lgpr}{{\sc lgp}\xspace}
\newcommand{\nusvr}{$\nu$-{\sc svr}\xspace}
\newcommand{\losvr}{{\sc l}o{\sc svr}\xspace}
\newcommand{\svr}{{\sc svr}\xspace}
\newcommand{\svm}{{\sc svm}\xspace}
\newcommand{\svms}{{\sc svm}s\xspace}
\newcommand{\lssvm}{{\sc ls-svm}\xspace}
\newcommand{\sogp}{{\sc sogp}\xspace}
\newcommand{\rfwr}{{\sc rfwr}\xspace}
\newcommand{\soms}{{\sc som}s\xspace}
\newcommand{\som}{{\sc som}\xspace}
\newcommand{\gpr}{{\sc gpr}\xspace}
\newcommand{\ema}{{\sc em}\xspace}
\newcommand{\ofl}{off-line\xspace}
\newcommand{\onl}{on-line\xspace}
\newcommand{\Ofl}{Off-line\xspace}
\newcommand{\Onl}{On-line\xspace}
\newcommand{\ofp}{off-policy\xspace}
\newcommand{\onp}{on-policy\xspace}
\newcommand{\td}{temporal difference\xspace}
\newcommand{\epse}{episodic policy search\xspace}
\newcommand{\epsa}{episodic-sample\xspace}
\newcommand{\epsas}{episodic-samples\xspace}
\newcommand{\ssa}{step-sample\xspace}
\newcommand{\rwa}{reward-weighted averaging\xspace}
\newcommand{\ssas}{step-samples\xspace}
\newcommand{\edas}{{\sc EDA}s\xspace}
\newcommand{\pse}{policy search\xspace}
\newcommand{\Pse}{Policy search\xspace}
\newcommand{\ngo}{natural gradient optimization\xspace}
\newcommand{\Ngo}{Natural gradient optimization\xspace}
\newcommand{\vgo}{vanilla gradient optimization\xspace}
\newcommand{\Vgo}{Vanilla gradient optimization\xspace}
\newcommand{\pid}{$\mathcal{PID}$\xspace}
\newcommand{\pd}{$\mathcal{PD}$\xspace}
\newcommand{\sqp}{{\sc sqp}\xspace}
\newcommand{\gep}{{\sc gep}\xspace}
\newcommand{\geps}{{\sc gep}s\xspace}
\newcommand{\qp}{{\sc qp}\xspace}
\newcommand{\roll}{rollout\xspace} % discount factor
\newcommand{\rolls}{rollouts\xspace} % discount factor

\newcommand{\robotcub}{{\sc RobotCub}\xspace}
\newcommand{\atr}{{\sc atr}\xspace}
\newcommand{\sarsa}{{\sc Sarsa}\xspace}
\newcommand{\ql}{{\sc q-learning}\xspace}
\newcommand{\barrett}{{\sc Barrett}\xspace}
\newcommand{\icub}{{\sc iCub}\xspace}
\newcommand{\james}{{\sc James}\xspace}

\newcommand{\mymath}[1]{\ensuremath{#1}\xspace}
\newcommand{\mymathbf}[1]{\mymath{\mathbf{\boldsymbol{#1}}}}
\newcommand{\covar}{\mymathbf{\Sigma}}
% \newcommand{\vtheta}{\mymathbf{\theta}}

\renewcommand{\vec}[1]{\mymathbf{#1}}
\newcommand{\mat}[1]{\mymathbf{#1}}
%\newcommand{\eps}{\vec{\epsilon}}

\newcommand{\varinit}{\mymath{\covar^{\mbox{\scriptsize init}}}}

% \newcommand{\mX}{\mat{X}}
% \newcommand{\mG}{\mat{G}}
% \newcommand{\mF}{\mat{F}}
% \newcommand{\vomega}{\vec{\omega}}
\newcommand{\Vomega}{\vec{\Omega}}
% \newcommand{\vs}{\vec{s}}
% \newcommand{\vo}{\vec{o}}
% \newcommand{\vu}{\vec{u}}
% \newcommand{\vx}{\vec{x}}
% \newcommand{\vw}{\vec{w}}
% \newcommand{\vj}{\vec{j}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\VO}{\mathcal{O}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\X}{\mathcal{X}}
% \newcommand{\E}{\mathcal{E}}
\newcommand{\T}{\mathcal{T}}

\newcommand{\f}{\mymath{f}}
\newcommand{\inpu}{\vec{\phi}}
\newcommand{\Inpu}{\mymath{\Phi}}
\newcommand{\vinpu}{\mymath{\tilde{\vec{\phi}}}}
\newcommand{\Vinpu}{\mymath{\tilde{\Phi}}}
\newcommand{\vnabla}{\mymath{\tilde{\nabla}_{\vinpu}}}
% \newcommand{\vf}{\mymath{\tilde{\f}}}

\newcommand{\hatf}{\mymath{\hat{\f}}}
\newcommand{\hatj}{\mymath{\hat{J}}}
\newcommand{\hatq}{\mymath{\hat{Q}}}
\newcommand{\hatv}{\mymath{\hat{V}}}
\newcommand{\hatu}{\mymath{\hat{U}}}

\newcommand{\her}{{\sc her}\xspace}
\newcommand{\gcp}{{\sc gcp}\xspace}
\newcommand{\gcps}{{\sc gcp}s\xspace}
\newcommand{\uvfa}{\textsc{uvfa}\xspace}
\newcommand{\uvfas}{{\sc uvfa}s\xspace}
\newcommand{\mtl}{{\sc mtl}\xspace}
\newcommand{\mrl}{{\sc mrl}\xspace}
\newcommand{\hrl}{{\sc hrl}\xspace}
\newcommand{\maml}{{\sc maml}\xspace}
\newcommand{\fomaml}{{\sc fomaml}\xspace}
\newcommand{\reptile}{{\sc reptile}\xspace}
\newcommand{\pearl}{{\sc pearl}\xspace}
\newcommand{\maesn}{{\sc maesn}\xspace}
\newcommand{\fr}{{\sc FetchReach}-v1\xspace}
\newcommand{\fp}{{\sc FetchPush}-v1\xspace}
\newcommand{\fs}{{\sc FetchSlide}-v1\xspace}
\newcommand{\fpap}{{\sc FetchPickAndPlace}-v1\xspace}
\newcommand{\fetch}{{\sc Fetch}\xspace}

\newcommand{\imgep}{\textsc{imgep}\xspace}
\newcommand{\fun}{{\sc f}u{\sc n}\xspace}
\newcommand{\darla}{{\sc darla}\xspace}
\newcommand{\distral}{{\sc distral}\xspace}
\newcommand{\unicorn}{{\sc unicorn}\xspace}
\newcommand{\saggriac}{{\sc sagg-riac}\xspace}
\newcommand{\iac}{{\sc iac}\xspace}
\newcommand{\ggan}{Goal{\sc gan}s\xspace}
\newcommand{\ogan}{Option{\sc gan}s\xspace}
\newcommand{\hdqn}{h-{\sc dqn}\xspace}
\newcommand{\hiro}{{\sc hiro}\xspace}
\newcommand{\asap}{{\sc asap}\xspace}
\newcommand{\rig}{{\sc rig}\xspace}
\newcommand{\hierq}{{\sc hierq}\xspace}
\newcommand{\hac}{{\sc hac}\xspace}
\newcommand{\hacob}{{\sc hacob}\xspace}
\newcommand{\ugl}{{\sc ugl}\xspace}
\newcommand{\mugl}{{\sc mugl}\xspace}
\newcommand{\diayn}{{\sc diayn}\xspace}
\newcommand{\discern}{{\sc discern}\xspace}
\newcommand{\curious}{{\sc curious}\xspace}
\newcommand{\imagine}{{\sc imagine}\xspace}
\newcommand{\decstr}{{\sc decstr}\xspace}
\newcommand{\archi}{{\sc lgb}\xspace}
\newcommand{\lArrowg}{{\sc l$\to$g}\xspace}
\newcommand{\lArrowb}{{\sc l$\to$b}\xspace}
\newcommand{\gArrowb}{{\sc g$\to$b}\xspace}
\newcommand{\lArrowgArrowb}{{\sc l$\to$g$\to$b}\xspace}
\newcommand{\lb}{{\sc lb}\xspace}
%\newcommand{\lg}{{\sc lg}\xspace}
\newcommand{\gb}{{\sc gb}\xspace}
\newcommand{\lgb}{{\sc lgb}\xspace}
\newcommand{\lgg}{{\sc lgg}\xspace}
\newcommand{\lcrl}{{\sc lc-rl}\xspace}
\newcommand{\gcrl}{{\sc gc-rl}\xspace}
\newcommand{\ai}{{\sc ai}\xspace}


\newcommand{\clic}{{\sc clic}\xspace}
\newcommand{\vic}{{\sc vic}\xspace}

\newcommand{\mt}{multitask\xspace}
\newcommand{\Mt}{Multitask\xspace}

\newcommand{\cs}{{\sc c}s\xspace}
\newcommand{\competence}{{\sc c}\xspace}
\newcommand{\lp}{{\sc lp}\xspace}
\newcommand{\proba}{{\sc p}\xspace}

\newcommand{\mujoco}{{\sc mujoco}\xspace}

\newcommand\wi[1]{$\circ$}
\newcommand\bu[1]{$\bullet$}
\newcommand\ot[1]{$\star$}
\newcommand\spa[1]{$\spadesuit$}
\newcommand\dn[1]{.}
\newcommand\no[1]{}
\newcommand\bo[1]{$\bullet\star$}

\newcommand\partielle[2]{\frac{\partial #1}{\partial #2}} % partial derivative

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1pt] (char) {\tiny #1};}}

\newcommand{\fk}{{$\mathcal{FK}$}\xspace}

%%% MDP and RL specific commands
\newcommand\pol{\pi} % policy
\newcommand\Pol{\Pi} % policy-space
\newcommand{\params}{{\mymathbf{\theta}}\xspace} % policy parameters (vector)
\newcommand{\Params}{\mymath{\Theta}}
\newcommand{\disc}{\gamma} % discount factor

\newenvironment{definition}{{\bf Definition:}}{\par}
\newenvironment{property}{{\bf Property:}}{\par}
\newenvironment{remark}{{\bf Remark:}}{\par}
\newenvironment{example}{{\bf Example:}}{\par}

\newcounter{cbox} \setcounter{cbox}{0}
\newcommand{\cbox}{\arabic{cbox}}
\newenvironment{mybox}[2]{\refstepcounter{cbox}\begin{tcolorbox}[title=Box \cbox: #1]\label{#2}\par}{\end{tcolorbox}}

\newcounter{cmes} \setcounter{cmes}{0}
\newcommand{\cmes}{\arabic{cmes}}
\newenvironment{mymes}[1]{\begin{tcolorbox}[colback=red!10!white]\refstepcounter{cmes}{\bf Message \cmes:}\label{#1}}{\end{tcolorbox}}

\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}[proposition]

\newtheorem{lemmaProof}{Proof of Lemma}
\newtheorem{propositionProof}{Proof of Proposition}
\newtheorem{corollaryProof}{Proof of Corollary}[propositionProof]

\usepackage{xcolor}
\definecolor{myred}{rgb}{0.8,0,0}
\definecolor{mypurple}{rgb}{0.6,0.22,0.8}

\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{myblue}{rgb}{0,0,0.7}
\definecolor{myindigo}{rgb}{0.4,0,0.7}
\newcommand{\note}[1]{\textcolor{myred}{\bf Note: {\em #1}}}
\newcommand{\biblio}[1]{\textcolor{myblue}{\fbox{\bf Todo:}{\em #1}}}

\newcommand{\todo}[1]{\textcolor{myred}{\fbox{\bf Todo:}{\em #1}}}
\newcommand{\ahmed}[1]{\textcolor{mypurple}{\fbox{\bf AA:}{#1}}}
\newcommand{\firas}[1]{\textcolor{myblue}{\fbox{\bf FJ:}{#1}}}

==> Source/Classical_RL.tex <==
\section{Reinforcement Learning in infinite horizon setting}
    Consider an infinite horizon Markov Decision Process (MDP) $\mathcal{M}=\{ \mathcal{S}, \mathcal{A}, \mathcal{P}, c, \gamma, p_0 \}$, where $\mathcal{S}$ and $\mathcal{A}$ are either finite or compact subsets of respectively $\mathbb{R}^d$ and $\mathbb{R}^{d'}$, $(d, d') \in \mathbb{N}^2$, $\mathcal{P}: \mathcal{S} \times \mathcal{A} \to \Delta(\mathcal{S})$ is a state transition kernel\footnote{$\Delta(\mathcal{S})$ denotes the set of probability measures over $\mathcal{S}$}, $c:\mathcal{S}\times \mathcal{A} \to \mathbb{R}$ is a continuous non-negative cost function, $p_0 \in \Delta(\mathcal{S})$ an initial state distribution and $\gamma \in (0,1)$ is the discount factor. 
    % \vspace{-0.3cm}
    % \begin{description}
    %     \item[--] $\mathcal{S}$ is either a finite or a compact subset of $\mathds{R}^d$, for some dimension $d\in \mathds{N}$
    %     \item[--] $\mathcal{A}$ is either a finite or a compact subset of $\mathds{R}^{d'}$, for $d' \in \mathds{N}$
    %     \item[--] $\mathcal{P}$ is the state transition kernel, i.e., a continuous mapping from $\mathcal{S} \times \mathcal{A}$ to $\Delta(\mathcal{S})$, where $\Delta(\cdot)$ denotes the set of probability measures\footnote{The $\sigma$-field is always the Borel one.} over some set,
    %     \item[--] $c:\mathcal{S}\times \mathcal{A} \to \mathbb{R}$ is a continuous non-negative cost function,
    %     \item[--] $p_0 \in \Delta(\mathcal{S})$ is the initial state distribution, and $\gamma \in (0,1)$ is the discount factor.
    % \end{description} 
    A policy $\pi$ is a mapping indicating, at each time step $t \in \mathbb{N}$, the action $a_t$ to be chosen at the current state  $s_t$. The goal of reinforcement learning algorithms is to optimise the discounted costs $\mathcal{L}(\pi, r) := \mathbb{E}_{\pi, p_0}\Big[ \sum_{t=0}^\infty \gamma^t c_t \Big], c_t := c(s_t,a_t)$,
    % \begin{align*}
    %     \mathcal{L}(\pi, r) := \mathbb{E}_{\pi, p_0}\Big[ \sum_{t=0}^\infty \gamma^t c_t \Big] \quad \textit{;} \quad  c_t := c(s_t,a_t)
    % \end{align*}
    where $\mathbb{E}_{\pi, p_0}$ denotes the expectation over trajectories generated in the MDP $\mathcal{M}$, using the policy $\pi$, and initialised according to $p_0$. 
    To this end, we look for a policy that achieves the optimal value function $V^*:\mathcal{S} \to \mathbb{R}$ defined as $V^*(s) = \min_{a_0, a_1, ... }\mathbb{E}_{\pi}\Big[\sum_{t=0}^\infty \gamma^t c_t \Big| s_0=s \Big]$. %and the state-action value function $Q^\pi:\mathcal{S}\times\mathcal{A} \to \mathbb{R}$ 
    % \begin{align*}
    %     V^*(s) = \min_{a_0, a_1, ... }\mathbb{E}_{\pi}\Big[\sum_{t=0}^\infty \gamma^t c_t \Big| s_0=s \Big]
    % \end{align*}
    
    The Bellman optimality principle suggests that it is possible to decomposes the optimisation into two sub problems: the current decision $(a_0)$ and all the remaining ones $(a_1,a_2,..)$. This translates into the following equation for any state $s_0\in\mathcal{S}$:
    \begin{align*}
        V^*(s_0) = \min_{a_0} \Big\{c(s_0,a_0) + \gamma \underbrace{\min_{a_1,a_2,...} \mathbb{E}_{\substack{s_{t+1}\sim \mathcal{P}(s_t,a_t)}}\Big[\sum_{t=1}^\infty \gamma^{t-1} c_t \Big]}_{\textstyle = \mathbb{E}_{s_1\sim \mathcal{P}(s_0,a_0)}[V^*(s_1)]} \Big\}
    \end{align*}
    a classical result in infinite horizon MDPs \cite{puterman2014markov} stipulates that if there exists a value function $V:\mathcal{S}\to\mathbb{R}$ and a policy $\pi^*:\mathcal{S}\to\mathcal{A}$ that verify the following:
    \begin{align}
        \pi^*(s) \in & \argmin_{a} \Big\{c(s,a) + \gamma \mathbb{E}_{s'\sim \mathcal{P}(s,a)}[V(s')] \Big\} \nonumber \\
        V(s) = & \min_{a} \Big\{c(s,a) + \gamma \mathbb{E}_{s'\sim \mathcal{P}(s,a)}[V(s')] \Big\} 
        \label{bellman-criterion}
    \end{align}
    then $\pi^*$ is an optimal control policy and $V=V^*=V^{\pi^*}$ where $V^{\pi}(s)$ is the expected discounted return of adopting the policy $\pi$ starting from the state $s$ defined as:
    \begin{align}
        V^{\pi}(s) = \mathbb{E}_{\pi, p_0}\Big[\sum_{t=0}^\infty \gamma^t c_t \Big| s_0=s \Big] = \mathbb{E}_{\substack{a\sim\pi(s) \\ s'\sim \mathcal{P}(s,a) }}\Big[c(s,a) + \gamma V^{\pi}(s')\Big].
        \label{V_bellman}
    \end{align}
    The Bellman criterion derived in Equation \eqref{bellman-criterion} proves that the optimal policy (in the sense of $\mathcal{L}$) is necessarily stationary: $\pi : \mathcal{S} \to \Delta(\mathcal{A})$.
    
    \subsection{Solving the geometrically discounted RL problem} 
        Value-based RL algorithms optimise $\mathcal{L}$ by looking for a policy that satisfies Equation \eqref{bellman-criterion}. This class of algorithm is grounded in the policy improvement theorem \cite{sutton2018reinforcement} that guarantees the construction of a better policy given the value function of a previous one. Let $\pi:\mathcal{S}\to\mathcal{A}$ be a given policy and let $V^\pi$ be the associated value function. Consider the policy $\hat{\pi}$ defined as: 
        \begin{align}
            \hat{\pi}(s) = \argmin_a \Big\{c(s,a) + \gamma \mathbb{E}_{s'\sim \mathcal{P}(s,a)}[V^\pi(s')] \Big\}.
            \label{policy_improvement}
        \end{align}
        The policy improvement theorem guarantees that $V^\pi(s) \leq V^{\hat{\pi}}(s)$ for any state $s\in\mathcal{S}$ \cite{sutton2018reinforcement}. 
        
        This principle is used in policy iteration (and even more recent algorithms such as Soft Actor Critic \cite{haarnoja2018soft}) to learn the optimal policy. Basically, the idea is to repeat the following steps up to convergence: 
        \begin{itemize}
            \item \textbf{Policy evaluation step:} Learn the value function $V^\pi$
            \item \textbf{Policy improvement step:} Update the policy according to Equation \eqref{policy_improvement} 
        \end{itemize}
        In order to learn the value function $V^\pi$, one possibility is to to iteratively apply of the Bellman operator $T_\pi$ (from $\mathbb{R}^{\mathcal{S}}$ to $\mathbb{R}^{\mathcal{S}}$) on a given value function $V: \mathcal{S} \to \mathbb{R}$. This operator is defined as:
        \begin{align*}
            [T_{\pi}(v)](s) = \mathbb{E}_{\substack{a\sim\pi(s) \\ s'\sim \mathcal{P}(s,a) }} \Big[c(s,a) + \gamma v(s') \Big],
        \end{align*}
        This approach is viable because $T_\pi$ is a $\gamma$-contraction whose unique solution is $V^\pi$.
        
    \subsection{The average-cost RL problem} 
        One way to avoid imposing the geometric discount is to consider the average-cost framework. In this setting the goal is to optimise the following objective function: 
        \begin{align*}
            \Bar{\mathcal{L}}(\pi,c) := \lim_{T\to\infty} \frac{1}{T} \mathbb{E}_{\pi, p_0}\Big[ \sum_{t=0}^T c_t \Big] 
        \end{align*}
        One possibility to optimise this criterion is to use a policy iteration scheme with a discount factor  $\gamma=1$. Naturally, the associated Bellman operator is no longer a contraction. For this reason, this approach is only guaranteed to work in specific MDP structure (such as reccurent MDPs). 
        
        In general, the average-cost problem can be viewer as the limit of the discounted RL problem. Notably, Blackwell proved that for any MDP, there exist a critical discount $\gamma_\text{crit}<1$ such that for any discount $\gamma\in(\gamma_\text{crit}, 1)$, solving the discounted problem is equivalent to solving the average cost one: 
        \begin{align*}
            \argmin_\pi \mathcal{L}(\pi,c) = \argmin_\pi \Bar{\mathcal{L}}(\pi,c) \quad \forall \gamma\in(\gamma_\text{crit}, 1)
        \end{align*}
        However, the critical discount $\gamma_\text{crit}$ can be arbitrarily close to 1 which induces major numerical instabilities in practice.  

==> Source/Limitations.tex <==
\section{Limitations}  
    Despite proving to be useful in order to solve hard exploration problems in tabular settings an improve sample efficiency in continuous environments, the proposed solutions of the delayed formulation admits several limitations 
    \paragraph{Theoretical limitations:}
        % policy improvement theorem 
        On the one hand, looking for the optimal stationary solution using Algorithm \ref{D-SAC}, the policy update does not guarantee a systematic improvement in the performance. 
        
        We found out in practice that this does not entail severe performance drawback 
        % Convergence bounds with respect to the horizon H
        
    \paragraph{Algorithmic limitations:}
        % Exploding value of the Q values 
        % increased computational burden 

==> Source/family_problems.tex <==
\section{Beyond the geometric discount}
    In order to reduce the bias against policies with longer mixing times without having to deal with numerical instabilities (by choosing a high discount factor) nor requiring a particular MDP structure (in order to explicitly solve the average cost formulation), we propose to solve the RL problem using a more flexible weighting distribution. 
    
    \subsection{A particular family of optimality criterion}
        For a given depth parameter $D\in\mathbb{N}$, we define the discount factors $\gamma_d \in(0,1)$ for any integer $d\in[0,D]$ and we consider the following optimality criterion:
        \begin{align}
            \mathcal{L}_D(\pi, c) := \mathbb{E}_{\pi, p_0} \Big[ \sum_{t=0}^\infty \Phi_D(t) c_t \Big] 
            \quad \textit{where} \quad 
            \Phi_D(t) := \sum_{\substack{ \{a_d \in \mathbb{N} \}_{i=0}^N \\ \textit{such that } \sum_d a_d = t  }} \quad \prod_{d=0}^N \gamma_d^{a_d}
        \end{align}
        
        
        \begin{wrapfigure}[15]{r}{0.5\textwidth}
            %\centering
            \includegraphics[width=0.5\textwidth]{Figures/Coefficents.png}
            \caption{\centering Cost weights over-time in $\mathcal{L}_D$}
        \label{fig:coefficents}
        \end{wrapfigure}
        
        This new criterion $\mathcal{L}_D$ puts more weights on future time steps which reduces the bias against policies with longer mixing time. This can be observed in Figure \ref{fig:coefficents} where we reported the normalised distribution of the weights $\Phi_D(t)$ obtained by setting the discount factors to the value $\gamma_d=0.99$. In fact, as $N$ increases, the mode of the probability distribution $\frac{\Phi_D(t)}{\sum_i \Phi_D(i)}$ is shifted toward the right, thus putting more weights on the future. 
        
        In addition, this class of optimality criterions can be seen as a generalisation of the classical geometric discount. In fact, we highlight that $\Phi_0(t) = \gamma_0^t$ which implies that $\mathcal{L}_0(\pi,c) = \mathcal{L}(\pi,c)$ for any policy $\pi$ and any cost function~$c$.
        
        In order to optimise this new criterion, we define the associated value functions:
        \begin{align*}
            V_D^\pi(s) := \mathbb{E}_{\pi} \Big[ \sum_{t=0}^\infty \Phi_D(t) c_t | s_0=s\Big] \; ; \;
            Q_D^\pi(s,a) := \mathbb{E}_{\pi} \Big[ \sum_{t=0}^\infty \Phi_D(t) c_t | s_0,a_0=s,a\Big]
        \end{align*}
        Similarly to the case of geometrically discounted RL (i.e. $D=0$), the obtained values functions are the fixed point of a particular operator that we derive in the following section.
        
    \subsection{Value functions are the unique fixed point of a Bellman like operator}
        To derive the desired operator, it is useful to derive a relationship between the coefficients~$\Phi_D(t)$: 
        \begin{Lemma}
            For any integer $D>0$ , the following equalities hold: 
            \begin{align*}
                \Phi_D(t) = \sum_{k=0}^t \gamma_D^k \Phi_{D-1}(t-k) = \Phi_{D-1}(t) + \gamma_D \Phi_D(t-1) = \sum_{d=0}^D \gamma_d \Phi_d(t-1)
            \end{align*}
            \label{L:weight_property}
        \end{Lemma}
        
        The latter equality in the previous lemma expresses the weight of the $t^\textit{th}$ cost in $\mathcal{L}_D$ as a linear combination of the weights of the previous time stamp ($t-1$) in $\mathcal{L}_{d}$ for $d\leq D$. This is used to establish the following relationship between the value functions $V_D^\pi(s)$ for any state $s\in\mathcal{S}$:
        \begin{proposition}
            For any state $s\in\mathcal{S}$ and for any integer $D\in\mathbb{N}$, we have:
            \begin{align*}
                V_D^\pi(s) = \mathbb{E}_{\substack{a\sim\pi(s) \\ s'\sim \mathcal{P}(s,a) }} \Big[c(s,a) + \sum_{d=0}^D \gamma_d V_d^\pi(s') \Big] 
            \end{align*}
            \label{P:value_decomposition}
        \end{proposition}
        Notably we can re-write the latter equality as: 
        \begin{align}
            V_D^\pi(s) = \underbrace{ \mathbb{E}_{\substack{a\sim\pi(s) \\ s'\sim \mathcal{P}(s,a) }} \Big[c(s,a) + \sum_{d=0}^{D-1} \gamma_d V_d^\pi(s') \Big]}_{\textstyle := c_D(s,a) } + \gamma_D \mathbb{E}_{\substack{a\sim\pi(s) \\ s'\sim \mathcal{P}(s,a) }} \Big[V_D^\pi(s')\Big]
            \label{bellman_V_d}
        \end{align}
        where $c_D(s,a)$ is an augmented cost function entirely defined through the MDP's cost function $c$ and the value functions $V_d^\pi$ for $d<D$. It ensues from this derivation that the value function $V_D^\pi$ is the unique fixed point of the following $\gamma_D$-contraction:
        \begin{align*}
            [T_{\pi}^D(v)](s) = \mathbb{E}_{\substack{a\sim\pi(s) \\ s'\sim \mathcal{P}(s,a) }} \Big[c_D(s,a) + \gamma_D v(s') \Big].
        \end{align*}
        A practical implication of this property is a tractable algorithmic approach to compute $V_D^\pi$ using any classical policy evaluation technique:
        \begin{algorithm}
            \caption{D-deep policy evaluation}\label{D-PE}
            \begin{algorithmic}[1]
                \STATE {\bfseries Input:} Depth parameter $D$, the cost function $c_0=c$, the policy $\pi$, the dynamics $\mathcal{P}$ (or \hbox{$\pi$-generated trajectories}), and a policy evaluation algorithm
                \FOR{$d \in [0, D]$}
                \STATE Evaluate $V_d^\pi$ using policy evaluation and the cost $c_d$ 
                \STATE Learn the cost $c_d(s,a) = \mathbb{E}_{\substack{a\sim\pi(s) \\ s'\sim \mathcal{P}(s,a) }} \Big[ c(s,a) + \sum_{i=0}^{d} \gamma_i V_i^\pi(s') \Big]$
                \ENDFOR
                \STATE {\bfseries Return:} $V_D^\pi$
            \end{algorithmic}
        \end{algorithm}
        Naturally, the latter algorithm can solve the problem exactly in tabular settings if the transition dynamics are provided. In more complex settings (continuous state/action space, unknown dynamics), sample-based policy evaluation techniques can be used to evaluate the third step and a supervised learning algorithm can be used to solve the fourth step. 
        
        We also point out that a similar reasoning can be applied to evaluate the Q-function associated to the $\mathcal{L}_D$ criterion. In fact, using Equation \eqref{bellman_V_d}, the following equality holds:
        \begin{align*}
            Q_D^\pi(s,a) = c(s,a) + \mathbb{E}_{s'\sim \mathcal{P}(s,a)}\Big[\sum_{d=0}^{D-1} \gamma_d V_d^\pi(s') \Big] + \gamma_D \mathbb{E}_{\substack{s'\sim \mathcal{P}(s,a) \\ a' \sim \pi(s')}}\Big[Q_D^\pi(s',a') \Big]
        \end{align*}
        
        This implies that $Q_D^\pi$ is also the unique fixed point of a $\gamma_D$-contraction. Practically it can be estimated with a similar scheme to the one presented in Algorithm \ref{D-PE}.
      

==> Source/optimal_planning.tex <==
\section{General non-geometrically discounted optimal decision making}
    In this section we discuss optimising a more general class of optimality criteria. Consider the following objective function: 
    \begin{align*}
        \mathcal{L}_{\eta}(\pi, c) := \mathbb{E}_{\pi, p_0}\Big[ \sum_t \eta(t) c_t \Big] \quad
        \textit{such that } \quad \eta(t) = \sum_{d=0}^D w_d \Phi_d(t)
    \end{align*}
    where the depth $D\in\mathbb{N}$ and the coefficients $w_d\in\mathbb{R}$ for any $d\in[0,D]$ are known. The weights $\Phi_d(t)$ are also computed using some predefined discounts $\gamma_d\in(0,1)$ for any $d\in[0,D]$. 
    
    This class of optimality criteria encapsulates in particular the geometrically discounted objective function. In fact setting $\eta = \Phi_0$ entails that $\mathcal{L}_\eta=\mathcal{L}_0=\mathcal{L}$.
    
    In this section, our goal is to provide a tractable approach to approximate the optimal sequence of actions that optimises $\mathcal{L}_\eta$. For this reason, we define the optimal value function as:
    \begin{align*}
        V_\eta^*(s) := \min_{a_{0:\infty}}\mathbb{E}_{a_{0:\infty}}\Big[\sum_{t=0}^\infty \eta(t) c_t | s_0=s\Big] \; ; \; Q_\eta^*(s,a) := \min_{a_{1:\infty}}\mathbb{E}_{a_{1:\infty}}\Big[\sum_{t=0}^\infty \eta(t) c_t | s_0,a_0=s,a\Big]
        %V_\eta^\pi(s) := \mathbb{E}_{\pi} \Big[ \sum_{t=0}^\infty \eta(t) c_t | s_0=s\Big] 
        %\; ; \; 
        %Q_\eta^\pi(s,a) := \mathbb{E}_{\pi} \Big[ \sum_{t=0}^\infty \eta(t) c_t | s_0,a_0=s,a\Big] 
    \end{align*}
    Where $\mathbb{E}_{a_0, a_1, ...}$ is the expectation over trajectories generated using the designated action profile. 
      
    \subsection{Optimal stationary policy}
        Given a stationary policy $\pi$, the associated value function in the sense of $\mathcal{L}_\eta$ can be decomposed into: 
        \begin{align}
            V_\eta^\pi(s) = \sum_{d=0}^D w_d V_d^\pi(s) \quad ; \quad Q_\eta^\pi(s,a) = \sum_{d=0}^D w_d Q_d^\pi(s,a)
            \label{value_linear_decomp}
        \end{align}
    
        In general, there is no guarantee that the optimal policy is stationary. However, the optimal stationary policy $\pi^*$ in the sense of $\mathcal{L}_\eta$ verifies $\pi^*(s) \in  \argmin_{a} Q_\eta^{\pi^*}(s,a)$ for any state $s\in \mathcal{S}$. For this reason, and similarly to policy evaluation algorithm, we propose to approximate the solution using the following two step procedure:
        \begin{itemize}
            \item \textbf{Policy evaluation step:} Evaluate $Q_\eta^{\pi_k}$ using deep-policy evaluation and Equation \eqref{value_linear_decomp}
            \item \textbf{Policy \st{improvement} update step:} Update the policy: $\pi_{k+1}(s)=\argmax_a Q_\eta^{\pi_k}(s,a)$
        \end{itemize}
        Unfortunately, the policy improvement theorem is no longer valid in this setting. For this reason, the proposed update rule does not guarantee a systematic improvement over the iterations. In practice, we noticed that the algorithm either converges to the optimal stationary policy, or gets stuck in a loop. 
        
        
    \subsection{Optimal decision making}
        The bellman optimality principle in this setting can be used to derive a relationship between $V_\eta^*$ and $V_{f(\eta)}^*$ where $f$ is an operator transforming the weighting distribution as follows: 
        \begin{align*}
            & \quad \Big[f(\eta)\Big](t) := \sum_{d=0}^D \big( \gamma_d \sum_{j=d}^D w_j \big) \Phi_d(t) = \langle\Gamma\cdot\Vec{w},\Vec{\Phi}(t)\rangle \\
            \textit{where } \quad & \Gamma := 
            \begin{bmatrix}
                \gamma_0 & \gamma_0 & \gamma_0 & ... & \gamma_0 \\
                0 & \gamma_1 & \gamma_1 & ... & \gamma_1 \\
                0 & 0 & \gamma_2 & ... & \gamma_2 \\
                \vdots & & & \ddots & \vdots \\
                0 & 0 & 0 & ... & \gamma_D 
            \end{bmatrix} \quad ; \quad
            \Vec{w}:= 
            \begin{bmatrix}
                w_0  \\
                w_1  \\
                w_2  \\
                \vdots \\
                w_D
            \end{bmatrix} \quad ; \quad
            \Vec{\Phi}(t):= 
            \begin{bmatrix}
                \Phi_0(t)  \\
                \Phi_1(t)  \\
                \Phi_2(t)  \\
                \vdots \\
                \Phi_D(t)
            \end{bmatrix} 
        \end{align*}
        The following proposition introduces the underlying relationship formally: 
        \begin{proposition}
            For any state $s_0\in\mathcal{S}$, the following identity holds: 
            \begin{align}
                V_\eta^*(s_0) = \min_{a_0} \Big\{ \big[\sum_{d=0}^D w_d\big] c(s_0,a_0) + \mathbb{E}_{s_1} \big[ V^*_{f(\eta)}(s_1) \big] \Big\}
                \label{bellman_general}
            \end{align}
            \label{P:bellman_general}
        \end{proposition}
        For the sake of simpler notations, let $\langle\Vec{1},\eta\rangle:=\sum_{d=0}^D w_d$ and let $\big[f^n(\eta)\big](t):=\langle\Gamma^n\cdot\Vec{w},\Vec{\Phi}(t)\rangle$  for any $n,t\in\mathbb{N}$. Using Equation \eqref{bellman_general} and an inductive reasoning w.r.t the horizon $H\in\mathbb{N}$ we get: 
        \begin{align}
            V_\eta^*(s_0) = \min_{a_{0:H}} \Big\{ \mathbb{E}_{a_{0:H}}\Big[\sum_{t=0}^H \langle\Vec{1},f^t(\eta)\rangle c_t\Big] + \mathbb{E}_{a_0,a_1,..,a_{H}} \big[ V^*_{f^{H+1}(\eta)}(s_{H+1}) \big] \Big\}
            \label{bellman_general_H}
        \end{align}
        As a consequence, the optimal policy in the sense of $\mathcal{L}_\eta$ is to execute the minimising arguments $a_{0:H}^*$ of Equation \eqref{bellman_general_H} and the execute the optimal policy in the sense $\mathcal{L}_{f^{H+1}(\eta)}$. Unfortunately, solving $\mathcal{L}_{f^{H+1}(\eta)}$ is not easier than the original problem. 
        
        However, under mild assumptions, for $H$ large enough, this criterion can be approximated with a simpler one. In order to derive this approximation, recall that the power iteration algorithm  described by the recurrence $\Vec{v}_{k+1}=\frac{\Gamma\cdot\Vec{v}_k}{\|\Gamma\cdot\Vec{v}_k\|}$ converges to the unit eigenvector corresponding to the largest eigenvalue of the matrix $\Gamma$ whenever that it is diagonalizable. In particular, if $0<\gamma_D<...<\gamma_0<1$ and $\Vec{v}_0=\Vec{w}$, then $\Gamma$ is diagonalizable, $\gamma_0$ is it's largest eigenvalue and the following holds:  
        \begin{align}
            \lim_{n\to\infty} \Vec{v}_{n+1} = \lim_{n\to\infty}\frac{\Gamma^n\cdot\Vec{w}}{\prod_{k\leq n}\|\Gamma\cdot\Vec{v}_k\|} = [\mathbb{1}_{i=0}]_{i\in[0,D]} 
            \quad \textit{and} \quad \lim_{n\to\infty}\frac{V^*_{f^n(\eta)}(s)}{\prod_{k\leq n}\|\Gamma\cdot\Vec{v}_k\|} = V^*(s)
            \label{bellman_asymptotic}
        \end{align}
        Under these premises, the right hand term of the minimisation problem in Equation~\eqref{bellman_general_H} can be approximated with the optimal value function in the sense of the classical RL criterion $\mathcal{L}$ (which optimal policy can be computed using any standard reinforcement learning algorithm in the literature). 
        
        Formally, we propose to approximate Equation \eqref{bellman_general_H} with a proxy optimal value function $\Tilde{V}_{\eta, H}^*(s_0)$:
        \begin{align}
            \Tilde{V}_{\eta, H}^*(s_0) = \min_{a_{0:H}} \Big\{ \mathbb{E}_{a_{0:H}}\Big[\sum_{t=0}^H \langle\Vec{1},f^t(\eta)\rangle c_t\Big] + \Big(\prod_{k\leq H}\|\Gamma\cdot\Vec{v}_k\|\Big) \mathbb{E}_{a_0,a_1,..,a_{H}} \big[ V^*(s_{H+1}) \big] \Big\}
            \label{approx_bellman_general_H}
        \end{align}
        A direct consequence of Equation \ref{bellman_asymptotic} is that $\lim_{H\to\infty}\Tilde{V}_{\eta, H}^*(s)=V_\eta^*(s)$ for any state $s\in\mathcal{S}$. In addition, for a given horizon $H$, the optimal decisions in the sense of the proxy problem formulation are to execute for the first $H$ steps the minimising arguments $a_{0:H}^*$ of Equation \eqref{approx_bellman_general_H} (they can be computed using dynamic programming) and then execute the optimal policy in the sense of the $\gamma_0$-discounted RL (which can be computed using any standard RL algorithm).
        
